Distribution Alignment: A Unified Framework for Long-tail Visual Recognition

Despite the recent success of deep neural networks, it remains challenging to effectively model the long-tail class distribution in visual recognition tasks. To address this problem, we first investigate the performance bottleneck of the two-stage learning framework via ablative study. Motivated by our discovery, we propose a unified distribution alignment strategy for long-tail visual recognition. Specifically, we develop an adaptive calibration function that enables us to adjust the classification scores for each data point. We then introduce a generalized re-weight method in the two-stage learning to balance the class prior, which provides a flexible and unified solution to diverse scenarios in visual recognition tasks. We validate our method by extensive experiments on four tasks, including image classification, semantic segmentation, object detection, and instance segmentation. Our approach achieves the state-of-the-art results across all four recognition tasks with a simple and unified framework. The code and models will be made publicly available at: https://github.com/Megvii-BaseDetection/DisAlign

==> sections/experiments_bak.tex <==
\section{Experiments}
In this section, we conduct a series of experiments to validate the effectiveness of our method. We evaluate our method on three visual recognition tasks, including image classification on ImageNet-LT dataset\cite{liu2019large}, object detection and instance segmentation on LVIS dataset\cite{gupta2019lvis}. In each task, we compare our approach to the state-of-the-art methods.

Below we present our experimental analysis on the ImageNet-LT dataset in Sec. \ref{subsec:classification}, followed by our results on LVIS dataset in Sec. \ref{subsec:lvis}. In each task, we first introduce the implementation details of our method, and then report the ablative study and comparisons of quantitative results on each dataset.



\subsection{Image Classification on ImageNet-LT}

\subsubsection{Experimental Details}
\paragraph{Datasets and Evaluation Metrics.} ImageNet-LT is a long-tail version of the original ImageNet-2012\cite{krizhevsky2012imagenet} first proposed in \cite{liu2019large}, which is generated by sampling a subset following the Parento distribution with the power value $\alpha=6$. It consists of 115.8K samples from 1000 categories, with maximally 1280 images per class and minimally 5 images per class. To demonstrate our method, we first report the \textit{top-1} and \textit{top-5} accuracy, and also calculate the accuracy of three disjoint subsets: \textit{many-shot classes}(classes each with over 100 training instances), \textit{medium-shot classes}(classes each with 20-100 training instances) and \textit{few-shot classes}(classes under 20 training instances).


\paragraph{Training Configuration.}
Following \cite{liu2019large}, we adopt the ResNet-10\cite{he2016deep} as the backbone network for feature extraction. 
%Different from the prior works\cite{liu2019large} that relies on two-stage training, our method jointly learns the instance feature, shared objcet class representations and downstream classification network. 
We initialize the parameters as in \cite{liu2019large} and train all the models from scratch. We use SGD with a mini-batch size of 256 and use the same learning rate scheduler with \cite{liu2019large}. We use a weight decay of 0.0001 and a momentum of 0.9. 


\begin{table*}[h!]

\centering
\caption{\textbf{Quantitative results on ImageNet-LT:} All models use the feature extractor trained with 90 epoch(except the models marked with \textbf{F-200e}, which means the feature extractors are trained with 200 epoch, $\dagger$ means the model uses cosine classifier. All our methods are reported with 95\% confidence interval over 10 runs.}
\vspace{-0.8em}
% \begin{threeparttable}
 \resizebox{0.99\textwidth}{!}{
\begin{tabular}{l|c|l|lll|l|lll}
\toprule
\multirow{2}{*}{\textbf{Method}}  & \multirow{2}{*}{\textbf{Align}} & \multicolumn{4}{c|}{\textbf{Top-1 Accuracy@R-50}} & \multicolumn{4}{c}{\textbf{Top-1 Accuracy@X-50}}  \\
\cmidrule{3-10}
                                  &             &\textbf{Average} & \textbf{Many } & \textbf{Medium } & \textbf{Few } &\textbf{Average} & \textbf{Many } & \textbf{Medium } & \textbf{Few } \\
\midrule
Naive\cite{kang2019decoupling}    & -           & 41.6	           & 64.0           &    33.8         &  5.8           & 44.4	          & 65.9           &       37.5     &  7.7 \\
%Cosine                            & -           & 48.4             &  68.4          &    41.8         &  15.2          & 49.2        &  68.9               &    42.8     & 15.6\\
\midrule
cRT\cite{kang2019decoupling}          & Learnable   & 47.3             & 58.8           &    44.0         &  26.1         &  49.6        & 61.8          &        46.2    &   27.4\\
cRT$^\dagger$                         & Learnable   & -                & -              &    -            &   -           &  49.7        & 60.4          &        46.8    &   29.3\\
LWS\cite{kang2019decoupling}          & Learnable   & 47.7             & 57.1           &    45.2         &  29.3         &  49.9        & 60.2          &        47.2    &   30.3  \\
NCM\cite{kang2019decoupling}          & Hand-Craft  & 44.3             & 53.1           &    42.3         &  26.5         & 47.3         & 56.6          &        45.3    &   28.1\\
$\tau$-Norm\cite{kang2019decoupling}  & Hand-Craft  & 46.7             & 56.6           &    44.2         &  27.4         & 49.4         & 59.1          &        46.9    &   30.7    \\
Logit Adjust\cite{}                   & Hand-Craft  & 50.3             & -              &      -          &   -           &            - & - &- &-\\
Deconfound$^\dagger$\cite{}           & Hand-Craft  &  -               & -              &      -          &   -           & 51.8            & 62.7       &        48.8    &   31.6\\
\midrule
%Naive$^\dagger$   & - & 45.2        &  67.4               &    38.0    & 7.5  \\
%Cosine$^\dagger$  & - & R-50 & 48.4        &  68.4               &    41.8    & 15.2   \\
%Naive-Bound                           &  -          & 56.1             & 62.3           &   53.6          & 47.6\\
\textbf{DisAlign}                     &  Learnable  &  51.29\colorpm{$\pm 0.03$}  &  59.90\colorpm{$\pm 0.04$} &  49.91\colorpm{$\pm 0.05$}  &  31.76\colorpm{$\pm 0.10$}      
                                                    &  52.49\colorpm{$\pm 0.03$}  &  61.54\colorpm{$\pm 0.03$} &  50.73\colorpm{$\pm 0.07$}  &  33.05\colorpm{$\pm 0.09$}\\
\textbf{DisAlign$^\dagger$}           &  Learnable  &  53.0 & 62.5 &  51.8 & 30.5 \\
\midrule
\textbf{DisAlign}\small(F-200e)      &  Learnable   &  53.68\colorpm{$\pm 0.03$} &   63.13\colorpm{$\pm 0.05$} &  51.46\colorpm{$\pm 0.06$}  &  34.74\colorpm{$\pm 0.08$}   \\
%\textbf{DisAlign$^\dagger$}\small(F-200e)   &  Learnable  &  \textbf{52.7} & 65.2 & \textbf{49.7} & 27.6 \\
%\midrule
%Naive$^\dagger$     & - & 45.2        &  67.4               &    38.0    & 7.5  \\
%
%Naive+SA$^\dagger$     & - & 48.4        &  68.4               &    41.7    & 15.5  \\
%\textbf{DisCal-Naive}  & & R-50 &  Learnable     &  51.7 & 62.3 & 48.7 & \textbf{32.1}   \\
%\textbf{DisCal-Cosine} & & R-50 &  Learnable  &  \textbf{52.7} & 65.2 & \textbf{49.7} & 27.6 \\
%\midrule
%cRT$^\dagger$\cite{kang2019decoupling}   & Learnable& 52.8   &   65.8  & 49.1 & 28.9  \\
%\textbf{DisCal-Naive}     &  Learnable   &  53.6 & 65.0 & 50.4 & \textbf{33.0}   \\
%\textbf{DisCal-Cosine}\small{(400e)} &  Learnable     & R-50  &  \textbf{52.8} & 65.2 & \textbf{49.8} & 28.0 \\
%\midrule
%Naive\cite{}  & X-50  & 44.4	             & 65.9               &          37.5        &  7.7   \\
%NCM\cite{}   & X-50  &   \\
%cRT\cite{}    & X-50       \\
%$\tau$-Norm\cite{} & X-50   
%LWS                & X-50     \\
%Deconfound-Cosine\cite{}         & X-50  &    \\
%Cosine\cite{} & X-50 & 47.6 & 67.3 & 41.3 & 14.0\\
%\midrule
%Naive$^\dagger$   & X-50     & 46.8        &  68.1               &    40.2    & 9.3   \\
%Cosine$^\dagger$  & X-50     & 49.2        &  68.9               &    42.8    & 15.6  \\
%\textbf{DisCal-Naive}   & X-50    & 52.3 & 62.6 & 49.6 & 32.8  \\
%\textbf{DisCal-Cosine}  & X-50    & 52.9 & 65.9 & 49.7 & 27.7\\
\bottomrule
 %\end{threeparttable}
\label{tab:classification}
\end{table*}


%
%\begin{table*}[h!]
%
%\centering
%\caption{\textbf{Quantitative results on ImageNet-LT:} The first block provides the comparisons with previous methods. The performance of \textbf{Plain Model$^\dagger$} reported in \cite{liu2019large} is trained only in 30 epochs. The \textbf{OLTR}$^\dagger$ \cite{liu2019large} is trained with \textbf{Resample}\cite{shen2016relay} in default. The second block of 5 rows shows the results of our re-implement baselines. For fair comparison, we report the performance of \textbf{Plain Model} which is trained with extra 60 epochs same with \cite{liu2019large}. The last block of 4 rows present the performance of re-balancing method equipped with our method and OLTR\cite{liu2019large}.}
%\vspace{-0.8em}
%% \begin{threeparttable}
% \resizebox{0.9\textwidth}{!}{
%\begin{tabular}{l|c|c|c|c|ccc}
%\toprule
%\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Epoch}} & \multirow{2}{*}{\textbf{Backbone}} & \multirow{2}{*}{\textbf{Post-Process}} & \multicolumn{4}{c}{\textbf{Top-1 Accuracy}}  \\
%\cmidrule{5-8}
%             & & & &  \textbf{Average} & \textbf{Many-shot} & \textbf{Medium-shot} & \textbf{Few-shot}   \\
%\midrule
%Naive\cite{kang2019decoupling} &\multirow{6}{*}{90}  & \multirow{6}{*}{R-50}  & -         & 41.6	             & 64.0               &          33.8        &  5.8  \\
%cRT\cite{kang2019decoupling}    &       & & Learnable & 47.3             & 58.8              &    44.0   & 26.1    \\
%LWS\cite{kang2019decoupling}    &    & & Learnable & 47.7        & 57.1              &    45.2   & 29.3   \\
%NCM\cite{kang2019decoupling}    &  & & Hand-Craft  & 44.3             & 53.1               &          42.3        &  26.5 \\
%$\tau$-Norm\cite{kang2019decoupling} & & & Hand-Craft   & 46.7        & 56.6              &    44.2   & 27.4    \\
%Logit Adjust(Post)\cite{} & & & Hand-Craft  & 50.3  & - &- &-\\
%%Logit Adjust(Loss)\cite{} & R-50 & 51.1  & - &- &-\\
%\midrule
%Naive$^\dagger$   & \multirow{3}{*}{90} & R-50 & - & 45.2        &  67.4               &    38.0    & 7.5  \\
%%Cosine$^\dagger$  & - & R-50 & 48.4        &  68.4               &    41.8    & 15.2   \\
%%Logit Adjust(Post)$^\dagger$\cite{} & Hand-Craft & R-50 & 50.8     &   62.8  & 48.6 & 24.9   \\
%%cRT$^\dagger$\cite{kang2019decoupling} & Learnable & R-50 & 50.8   &   62.2  & 47.7 & 29.1  \\
%
%%\textbf{DisCal-Naive}(Non-parametric) & R-50  &    \\
%\textbf{DisCal-Naive}  & & R-50 &  Learnable     &  51.7 & 62.3 & 48.7 & \textbf{32.1}   \\
%\textbf{DisCal-Cosine} & & R-50 &  Learnable  &  \textbf{52.7} & 65.2 & \textbf{49.7} & 27.6 \\
%\midrule
%Naive$^\dagger$   & \multirow{2}{*}{90} & R-50 & - & 45.2        &  67.4               &    38.0    & 7.5  \\
%
%Naive+SA$^\dagger$   &   & R-50 & - & 48.4        &  68.4               &    41.7    & 15.5  \\
%%\textbf{DisCal-Naive}  & & R-50 &  Learnable     &  51.7 & 62.3 & 48.7 & \textbf{32.1}   \\
%%\textbf{DisCal-Cosine} & & R-50 &  Learnable  &  \textbf{52.7} & 65.2 & \textbf{49.7} & 27.6 \\
%\midrule
%cRT$^\dagger$\cite{kang2019decoupling} & \multirow{2}{*}{400} & R-50  & Learnable& 52.8   &   65.8  & 49.1 & 28.9  \\
%\textbf{DisCal-Naive} &     & R-50 &  Learnable   &  53.6 & 65.0 & 50.4 & \textbf{33.0}   \\
%%\textbf{DisCal-Cosine}\small{(400e)} &  Learnable     & R-50  &  \textbf{52.8} & 65.2 & \textbf{49.8} & 28.0 \\
%\midrule
%Naive\cite{}  & X-50 &    & 44.4	             & 65.9               &          37.5        &  7.7   \\
%NCM\cite{}   & X-50  &    & 47.3              & 56.6               &          45.3        &  28.1  \\
%cRT\cite{}    & X-50 &   &  49.6              & 61.8               &          46.2   &     27.4    \\
%$\tau$-Norm\cite{} & X-50 &    & 49.4         & 59.1               &          46.9   &     30.7    \\
%LWS                & X-50  &    & 49.9        & 60.2               &          47.2   &     30.3    \\
%Deconfound-Cosine\cite{}         & X-50  &    & 51.8        & 62.7               &          48.8  &  31.6 \\
%Cosine\cite{} & X-50 & & 47.6 & 67.3 & 41.3 & 14.0\\
%\midrule
%Naive$^\dagger$   & X-50  &    & 46.8        &  68.1               &    40.2    & 9.3   \\
%Cosine$^\dagger$  & X-50  &    & 49.2        &  68.9               &    42.8    & 15.6  \\
%\textbf{DisCal-Naive}   & X-50      &  & 52.3 & 62.6 & 49.6 & 32.8  \\
%\textbf{DisCal-Cosine}  & X-50  &   & 52.9 & 65.9 & 49.7 & 27.7\\
%\bottomrule
%\end{tabular}}
%%\end{threeparttable}
%\label{tab:classification}
%\end{table*}
%


\subsection{Semantic Semgnetaion on ADE20k Dataset}

\begin{table*}[h!]

\centering
\caption{\textbf{Results on ADE-20K:} All baseline models are trained with a image size of 512x512 and 160K iteration in total.}
\vspace{-0.8em}
% \begin{threeparttable}
 \resizebox{0.999\textwidth}{!}{
\begin{tabular}{l|c||l|lll||l|lll}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{B}} & \multicolumn{4}{c||}{\textbf{Mean IoU}} & \multicolumn{4}{c}{\textbf{Mean Accuracy}}\\
\cmidrule{3-10}
              & & \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} &  \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} \\
\midrule

%% FCN with Res-50
%FCN\cite{kang2019decoupling}  &\multirow{4}{*}{R-50} & \xmark & 36.1  &  62.5   &  38.1   & 27.6 
%															  & 45.4  &  76.9   &  48.8   & 34.5 \\
%\textbf{FCN+DisAlign}          &                     & \xmark & 37.5\more{(+1.4)}  & 62.6\more{(+0.1)}  & 40.2\more{(+2.1)} & 28.8\more{(+1.2)} 
%															  & 49.9\more{(+4.5)}  & 76.7\small{(-0.2)} & 54.2\more{(+5.3)} & 39.2\more{(+4.7)}\\
FCN\cite{kang2019decoupling}  & \multirow{2}{*}{R-50}    & 38.1  &  64.6   &  40.0   & 29.6 
															  & 46.3  &  78.6   &  49.3   & 35.4 \\
\textbf{FCN+DisAlign}         &                       & 40.1\more{(+2.0)}  & 65.0\more{(+0.4)}  & 42.8\more{(+2.6)} & 31.3\more{(+2.5)}   
															  & 51.4\more{(+5.1)}  & 78.6\small{(+0.0)} & 56.1\more{(+5.8)} & 40.6\more{(+5.2)}\\
\midrule%% FCN with Res-101
%FCN\cite{kang2019decoupling}  &\multirow{4}{*}{R-101} & \xmark &  39.9  &  65.3   &  42.0   & 31.7 
%															   &  49.6  &  79.1   &  52.6   & 39.6 \\
%\textbf{FCN+DisAlign}          &   &\xmark                     &  41.8\more{(+1.9)}  &  65.5\more{(+0.2)}   & 44.1\more{(+2.1)}  & 33.8\more{(+2.1)}  % on V100
%                                                               &  54.7\more{(+5.1)}  &  79.0\small{(-0.1)}  & 58.7\more{(+6.1)}  & 45.3\more{(+5.7)}\\
FCN\cite{kang2019decoupling}  &  \multirow{2}{*}{R-101}     &  41.4  &   67.0  &  43.3   & 33.2 
																   &  50.2  &   80.6  &  52.9   & 40.1 \\
\textbf{FCN+DisAlign}         &                            &  43.7\more{(+2.3)}  & 67.4\more{(+0.4)}  & 46.1\more{(+2.8)} & 35.7\more{(+2.5)}   
														           &  55.9\more{(+5.7)}  & 80.6\small{(+0.0)} & 59.7\more{(+4.8)} & 46.4\more{(+6.3)}  \\
\midrule

%% FCN with Res-101
%FCN\cite{kang2019decoupling}  &\multirow{4}{*}{S-101} & \xmark  & 45.6  &  66.6  &  47.5   & 38.6 
%																& 57.8  &  79.8  &  62.1   & 48.9 \\
%\textbf{FCN+DisAlign}        &                        & \xmark  & 46.2\more{(+0.6)}  & 66.6\small{(+0.0)}   & 47.9\more{(+0.4)}    & 39.4\more{(+0.8)}   
%																& 60.4\more{(+1.6)}  & 79.0\small{(-0.8)}& 64.9\more{(+2.8)} & 51.7\more{(+2.8)}\\
FCN\cite{kang2019decoupling}  &  \multirow{2}{*}{S-101}          & 46.2  & 67.6   & 48.0  & 39.1 
																	  & 57.3  & 79.4   & 61.7  & 48.2   \\
\textbf{FCN+DisAlign}         &                              & 46.9\more{(+0.7)}  & 67.7\more{(+0.1)}  & 48.2\more{(+0.2)}  & 40.3\more{(+1.2)}
																      & 60.1\more{(+2.8)} &  79.7\more{(+0.3)}  & 64.2\more{(+2.5)}  & 51.9\more{(+3.7)} \\
\midrule
\midrule
%% PSPNet with Res-101
%PSPNet\cite{kang2019decoupling}  &\multirow{4}{*}{R-101}  & \xmark & 44.4  & 66.9   & 46.6    & 36.8  & 54.7 & 79.7 & 58.7 & 45.2 \\
%\textbf{PSPNet+DisAlign}   &  &\xmark                              &   &    &     &    & \\
%PSPNet\cite{kang2019decoupling}  &  & \cmark                       & 45.35  &     &    &  & \\
%\textbf{PSPNet+DisAlign}   &        & \cmark                       &        &     &    &  & \\
%\midrule

%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{4}{*}{R-50} & \xmark  &  43.9  &  66.6  &   47.1  &   35.6 
%																		  &  54.9  &  79.4  &   60.3  &   44.5     \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \xmark &  44.4\more{(+0.5)} & 66.6\small{(+0.0)} & 47.2\more{(+0.1)} & 36.5\more{(+0.9)} 
%																		  &  56.9\more{(+2.0)} & 79.9\more{(+0.5)}  & 62.2\more{(+1.9)} & 46.9\more{(+2.4)} \\
DeepLabV3$^{+}$\cite{kang2019decoupling} & \multirow{2}{*}{R-50}   &  44.9  &  67.7  &   48.3  &   36.4 
																		  &  55.0  &  80.1  &   60.8  &   44.1 \\
\textbf{DeepLabV3$^{+}$+DisAlign}        &                        &  45.7\more{(+0.8)} & 67.7\small{(+0.0)} & 48.6\more{(+0.3)} & 37.8\more{(+1.4)}
																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
\midrule
%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{4}{*}{R-101} & \xmark &  45.5 & 67.6 & 48.2 & 37.6 & 56.5 & 80.0 & 61.2 & 46.6     \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \xmark &  46.0\more{(+0.5)} & 67.6\small{(+0.0)} & 48.4\more{(+0.2)} & 38.5\more{(+0.9)} 
%																		  &  59.1\more{(+2.6)} & 80.5\more{(+0.5)} & 63.8\more{(+2.6)} & 49.9\more{(+3.3)} \\
DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{2}{*}{R-101}  &  46.4 & 68.7  & 49.0 & 38.4 & 56.7 & 80.9 & 61.5 & 47.7 \\
\textbf{DeepLabV3$^{+}$+DisAlign}        &                        &  47.1\more{(+0.7)} & 68.7\small{(+0.0)} & 49.4\more{(+0.4)} & 39.6\more{(+1.2)}
																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
\midrule
%% PSPNet with Res-101
%PSPNet\cite{kang2019decoupling}  &\multirow{4}{*}{S-101}  & \xmark & 45.4 & 67.1 & 48.1  & 37.7 & 56.9 & 79.4 & 61.7 & 47.4 \\
%\textbf{PSPNet+DisAlign}   &  &\xmark                              &   &    &     &    & \\
%PSPNet\cite{kang2019decoupling}  &  & \cmark                       & 46.3  &     &    &  & \\
%\textbf{PSPNet+DisAlign}   &        & \cmark                       &        &     &    &  & \\
%\midrule
%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{4}{*}{S-101} & \xmark   &  46.5  & 68.0  & 49.1 & 38.8 
%																			&  58.1  & 80.1  & 63.4 & 48.4     \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \xmark   &  46.9\more{(+0.4)} & 67.8\small{(-0.2)} & 49.2\more{(+0.1)} & 39.6\more{(+0.8)} % on V100
%																		    &  60.8\more{(+2.7)} & 80.3\more{(+0.2)}  & 65.5\more{(+2.1)}  & 52.2\more{(+3.8)}\\

DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{2}{*}{S-101}  &  47.3 & 69.0 & 49.7 & 39.7
																	      &  58.1 & 80.8 & 63.4 & 48.2\\
\textbf{DeepLabV3$^{+}$+DisAlign}        &                       &  47.8\more{(+0.5)} & 68.9\small{(-0.1)} & 49.8\more{(+0.1)} & 40.7\more{(+1.0)} 
																		  &  60.1\more{(+2.0)} & 81.0\more{(+0.2)}  & 65.5\more{(+2.1)} & 52.0\more{(+1.8)}\\
\midrule
\bottomrule
\end{tabular}}
\label{tab:classification}
\end{table*}


%
% Backup
%\begin{table*}[h!]
%
%\centering
%\caption{\textbf{Results on ADE-20K:} All baseline models are trained with a image size of 512x512 and 160K iteration in total.}
%\vspace{-0.8em}
%% \begin{threeparttable}
% \resizebox{0.999\textwidth}{!}{
%\begin{tabular}{l|c||c|l|lll||l|lll}
%\toprule
%\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{B}} & \multirow{2}{*}{\textbf{Aug}} & \multicolumn{4}{c||}{\textbf{Mean IoU}} & \multicolumn{4}{c}{\textbf{Mean Accuracy}}\\
%\cmidrule{4-10}
%              & & & \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} &  \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} \\
%\midrule
%
%%% FCN with Res-50
%FCN\cite{kang2019decoupling}  &\multirow{4}{*}{R-50} & \xmark & 36.1  &  62.5   &  38.1   & 27.6 
%															  & 45.4  &  76.9   &  48.8   & 34.5 \\
%\textbf{FCN+DisAlign}          &                     & \xmark & 37.5\more{(+1.4)}  & 62.6\more{(+0.1)}  & 40.2\more{(+2.1)} & 28.8\more{(+1.2)} 
%															  & 49.9\more{(+4.5)}  & 76.7\small{(-0.2)} & 54.2\more{(+5.3)} & 39.2\more{(+4.7)}\\
%FCN\cite{kang2019decoupling}  &                      & \cmark & 38.1  &  64.6   &  40.0   & 29.6 
%															  & 46.3  &  78.6   &  49.3   & 35.4 \\
%\textbf{FCN+DisAlign}         &                      & \cmark & 40.1\more{(+2.0)}  & 65.0\more{(+0.4)}  & 42.8\more{(+2.6)} & 31.3\more{(+2.5)}   
%															  & 51.4\more{(+5.1)}  & 78.6\small{(+0.0)} & 56.1\more{(+5.8)} & 40.6\more{(+5.2)}\\
%\midrule%% FCN with Res-101
%FCN\cite{kang2019decoupling}  &\multirow{4}{*}{R-101} & \xmark &  39.9  &  65.3   &  42.0   & 31.7 
%															   &  49.6  &  79.1   &  52.6   & 39.6 \\
%\textbf{FCN+DisAlign}          &   &\xmark                     &  41.8\more{(+1.9)}  &  65.5\more{(+0.2)}   & 44.1\more{(+2.1)}  & 33.8\more{(+2.1)}  % on V100
%                                                               &  54.7\more{(+5.1)}  &  79.0\small{(-0.1)}  & 58.7\more{(+6.1)}  & 45.3\more{(+5.7)}\\
%FCN\cite{kang2019decoupling}  &                           & \cmark &  41.4  &   67.0  &  43.3   & 33.2 
%																   &  50.2  &   80.6  &  52.9   & 40.1 \\
%\textbf{FCN+DisAlign}         &                           & \cmark &  43.7\more{(+2.3)}  & 67.4\more{(+0.4)}  & 46.1\more{(+2.8)} & 35.7\more{(+2.5)}   
%														           &  55.9\more{(+5.7)}  & 80.6\small{(+0.0)} & 59.7\more{(+4.8)} & 46.4\more{(+6.3)}  \\
%\midrule
%
%%% FCN with Res-101
%FCN\cite{kang2019decoupling}  &\multirow{4}{*}{S-101} & \xmark  & 45.6  &  66.6  &  47.5   & 38.6 
%																& 57.8  &  79.8  &  62.1   & 48.9 \\
%\textbf{FCN+DisAlign}        &                        & \xmark  & 46.2\more{(+0.6)}  & 66.6\small{(+0.0)}   & 47.9\more{(+0.4)}    & 39.4\more{(+0.8)}   
%																& 60.4\more{(+1.6)}  & 79.0\small{(-0.8)}& 64.9\more{(+2.8)} & 51.7\more{(+2.8)}\\
%FCN\cite{kang2019decoupling}  &                             & \cmark  & 46.2  & 67.6   & 48.0  & 39.1 
%																	  & 57.3  & 79.4   & 61.7  & 48.2   \\
%\textbf{FCN+DisAlign}         & & \cmark                              & 46.9\more{(+0.7)}  & 67.7\more{(+0.1)}  & 48.2\more{(+0.2)}  & 40.3\more{(+1.2)}
%																      & 60.1\more{(+2.8)} &  79.7\more{(+0.3)}  & 64.2\more{(+2.5)}  & 51.9\more{(+3.7)} \\
%\midrule
%\midrule
%%% PSPNet with Res-101
%%PSPNet\cite{kang2019decoupling}  &\multirow{4}{*}{R-101}  & \xmark & 44.4  & 66.9   & 46.6    & 36.8  & 54.7 & 79.7 & 58.7 & 45.2 \\
%%\textbf{PSPNet+DisAlign}   &  &\xmark                              &   &    &     &    & \\
%%PSPNet\cite{kang2019decoupling}  &  & \cmark                       & 45.35  &     &    &  & \\
%%\textbf{PSPNet+DisAlign}   &        & \cmark                       &        &     &    &  & \\
%%\midrule
%
%%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{4}{*}{R-50} & \xmark  &  43.9  &  66.6  &   47.1  &   35.6 
%																		  &  54.9  &  79.4  &   60.3  &   44.5     \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \xmark &  44.4\more{(+0.5)} & 66.6\small{(+0.0)} & 47.2\more{(+0.1)} & 36.5\more{(+0.9)} 
%																		  &  56.9\more{(+2.0)} & 79.9\more{(+0.5)}  & 62.2\more{(+1.9)} & 46.9\more{(+2.4)} \\
%DeepLabV3$^{+}$\cite{kang2019decoupling} &                       & \cmark &  44.9  &  67.7  &   48.3  &   36.4 
%																		  &  55.0  &  80.1  &   60.8  &   44.1 \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \cmark &  45.7\more{(+0.8)} & 67.7\small{(+0.0)} & 48.6\more{(+0.3)} & 37.8\more{(+1.4)}
%																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
%\midrule
%%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{4}{*}{R-101} & \xmark &  45.5 & 67.6 & 48.2 & 37.6 & 56.5 & 80.0 & 61.2 & 46.6     \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \xmark &  46.0\more{(+0.5)} & 67.6\small{(+0.0)} & 48.4\more{(+0.2)} & 38.5\more{(+0.9)} 
%																		  &  59.1\more{(+2.6)} & 80.5\more{(+0.5)} & 63.8\more{(+2.6)} & 49.9\more{(+3.3)} \\
%DeepLabV3$^{+}$\cite{kang2019decoupling} &                       & \cmark &  46.4 & 68.7  & 49.0 & 38.4 & 56.7 & 80.9 & 61.5 & 47.7 \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \cmark &  47.1\more{(+0.7)} & 68.7\small{(+0.0)} & 49.4\more{(+0.4)} & 39.6\more{(+1.2)}
%																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
%\midrule
%%% PSPNet with Res-101
%%PSPNet\cite{kang2019decoupling}  &\multirow{4}{*}{S-101}  & \xmark & 45.4 & 67.1 & 48.1  & 37.7 & 56.9 & 79.4 & 61.7 & 47.4 \\
%%\textbf{PSPNet+DisAlign}   &  &\xmark                              &   &    &     &    & \\
%%PSPNet\cite{kang2019decoupling}  &  & \cmark                       & 46.3  &     &    &  & \\
%%\textbf{PSPNet+DisAlign}   &        & \cmark                       &        &     &    &  & \\
%%\midrule
%%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{4}{*}{S-101} & \xmark   &  46.5  & 68.0  & 49.1 & 38.8 
%																			&  58.1  & 80.1  & 63.4 & 48.4     \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \xmark   &  46.9\more{(+0.4)} & 67.8\small{(-0.2)} & 49.2\more{(+0.1)} & 39.6\more{(+0.8)} % on V100
%																		    &  60.8\more{(+2.7)} & 80.3\more{(+0.2)}  & 65.5\more{(+2.1)}  & 52.2\more{(+3.8)}\\
%%Scope                 mIoU       mAcc       aAcc
%%global               47.27      58.08      82.51
%%LongTail:
%%Head                 69.03      80.75
%%Body                 49.68      63.37
%%Tail                 39.69      48.16
%
%DeepLabV3$^{+}$\cite{kang2019decoupling} &                       & \cmark &  47.3 & 69.0 & 49.7 & 39.7
%																	      &  58.1 & 80.8 & 63.4 & 48.2\\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \cmark &  47.8\more{(+0.5)} & 68.9\small{(-0.1)} & 49.8\more{(+0.1)} & 40.7\more{(+1.0)} 
%																		  &  60.1\more{(+2.0)} & 81.0\more{(+0.2)}  & 65.5\more{(+2.1)} & 52.0\more{(+1.8)}\\
%\midrule
%\bottomrule
%\end{tabular}}
%\label{tab:classification}
%\end{table*}

%
%\begin{table*}[h!]
%
%\centering
%\caption{\textbf{Results on ADE-20K:} All baseline models are trained with a image size of 512x512 and 160K iteration in total.}
%\vspace{-0.8em}
%% \begin{threeparttable}
% \resizebox{0.999\textwidth}{!}{
%\begin{tabular}{l|c||c|l|lll||l|lll}
%\toprule
%\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{B}} & \multirow{2}{*}{\textbf{Aug}} & \multicolumn{4}{c||}{\textbf{Mean IoU}} & \multicolumn{4}{c}{\textbf{Mean Accuracy}}\\
%\cmidrule{4-10}
%              & & & \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} &  \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} \\
%\midrule
%
%%% FCN with Res-50
%FCN\cite{kang2019decoupling}  &\multirow{4}{*}{R-50} & \xmark & 36.1  &  62.5   &  38.1   & 27.6 
%															  & 45.4  &  76.9   &  48.8   & 34.5 \\
%\textbf{FCN+DisAlign}          &                     & \xmark & 37.5\more{(+1.4)}  & 62.6\more{(+0.1)}  & 40.2\more{(+2.1)} & 28.8\more{(+1.2)} 
%															  & 49.9\more{(+4.5)}  & 76.7\small{(-0.2)} & 54.2\more{(+5.3)} & 39.2\more{(+4.7)}\\
%FCN\cite{kang2019decoupling}  &                      & \cmark & 38.1  &  64.6   &  40.0   & 29.6 
%															  & 46.3  &  78.6   &  49.3   & 35.4 \\
%\textbf{FCN+DisAlign}         &                      & \cmark & 40.1\more{(+2.0)}  & 65.0\more{(+0.4)}  & 42.8\more{(+2.6)} & 31.3\more{(+2.5)}   
%															  & 51.4\more{(+5.1)}  & 78.6\small{(+0.0)} & 56.1\more{(+5.8)} & 40.6\more{(+5.2)}\\
%\midrule%% FCN with Res-101
%FCN\cite{kang2019decoupling}  &\multirow{4}{*}{R-101} & \xmark &  39.9  &  65.3   &  42.0   & 31.7 & 49.6 & 79.1 & 52.6 & 39.6 \\
%\textbf{FCN+DisAlign}          &   &\xmark                       &    &     &      &   & \\
%FCN\cite{kang2019decoupling}  &                            & \cmark &  41.4  &   67.0  &  43.3   & 33.2 & 50.2 & 80.6 & 52.9 & 40.1 \\
%\textbf{FCN+DisAlign}         & & \cmark                  &      &      &     &    & \\
%\midrule
%
%%% FCN with Res-101
%FCN\cite{kang2019decoupling}  &\multirow{4}{*}{S-101} & \xmark  & 45.6  &  66.6  &  47.5   & 38.6 & 57.8 & 79.8 & 62.1 & 48.9 \\
%\textbf{FCN+DisAlign}        &   &\xmark                       &    &     &      &   & \\
%FCN\cite{kang2019decoupling}  &                             & \cmark  & 46.2  &      &    &   & \\
%\textbf{FCN+DisAlign}         & & \cmark                    &      &      &     &    & \\
%\midrule
%%% PSPNet with Res-101
%%PSPNet\cite{kang2019decoupling}  &\multirow{4}{*}{R-101}  & \xmark & 44.4  & 66.9   & 46.6    & 36.8  & 54.7 & 79.7 & 58.7 & 45.2 \\
%%\textbf{PSPNet+DisAlign}   &  &\xmark                              &   &    &     &    & \\
%%PSPNet\cite{kang2019decoupling}  &  & \cmark                       & 45.35  &     &    &  & \\
%%\textbf{PSPNet+DisAlign}   &        & \cmark                       &        &     &    &  & \\
%%\midrule
%
%%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{4}{*}{R-50} & \xmark  &  43.9  &  66.6  &   47.1  &   35.6 
%																		  &  54.9  &  79.4  &   60.3  &   44.5     \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \xmark &  44.4\more{(+0.5)} & 66.6\small{(+0.0)} & 47.2\more{(+0.1)} & 36.5\more{(+0.9)} 
%																		  &  56.9\more{(+2.0)} & 79.9\more{(+0.5)}  & 62.2\more{(+1.9)} & 46.9\more{(+2.4)} \\
%DeepLabV3$^{+}$\cite{kang2019decoupling} &                       & \cmark &  44.9  &  67.7  &   48.3  &   36.4 
%																		  &  55.0  &  80.1  &   60.8  &   44.1 \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \cmark &  45.7\more{(+0.8)} & 67.7\small{(+0.0)} & 48.6\more{(+0.3)} & 37.8\more{(+1.4)}
%																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
%\midrule
%%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{4}{*}{R-101} & \xmark &  45.5 & 67.6 & 48.2 & 37.6 & 56.5 & 80.0 & 61.2 & 46.6     \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \xmark &  46.0\more{(+0.5)} & 67.6\small{(+0.0)} & 48.4\more{(+0.2)} & 38.5\more{(+0.9)} 
%																		  &  59.1\more{(+2.6)} & 80.5\more{(+0.5)} & 63.8\more{(+2.6)} & 49.9\more{(+3.3)} \\
%DeepLabV3$^{+}$\cite{kang2019decoupling} &                       & \cmark &  46.4 & 68.7  & 49.0 & 38.4 & 56.7 & 80.9 & 61.5 & 47.7 \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \cmark &  47.1\more{(+0.7)} & 68.7\small{(+0.0)} & 49.4\more{(+0.4)} & 39.6\more{(+1.2)}
%																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
%\midrule
%%% PSPNet with Res-101
%%PSPNet\cite{kang2019decoupling}  &\multirow{4}{*}{S-101}  & \xmark & 45.4 & 67.1 & 48.1  & 37.7 & 56.9 & 79.4 & 61.7 & 47.4 \\
%%\textbf{PSPNet+DisAlign}   &  &\xmark                              &   &    &     &    & \\
%%PSPNet\cite{kang2019decoupling}  &  & \cmark                       & 46.3  &     &    &  & \\
%%\textbf{PSPNet+DisAlign}   &        & \cmark                       &        &     &    &  & \\
%%\midrule
%%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{4}{*}{S-101} & \xmark   &  46.5  & 68.0  & 49.1 & 38.8 
%																			&  58.1  & 80.1  & 63.4 & 48.4     \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \xmark   &  46.8\more{(+0.3)} & 67.8\small{(-0.2)} & 49.1\small{(+0.0)} & 39.5\more{(+1.5)}
%																		    &  60.7\more{(+2.6)} & 80.4\more{(+0.3)}  & 65.6\more{(+2.2)}  & 51.9\more{(+3.5)}\\
%DeepLabV3$^{+}$\cite{kang2019decoupling} &                       & \cmark &  47.3 &   & \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       & \cmark & \\
%\midrule
%\bottomrule
%\end{tabular}}
%\label{tab:classification}
%\end{table*}



%
%
%\begin{table*}[h!]
%
%\centering
%\caption{\textbf{Quantitative results on ImageNet-LT:} The first block provides the comparisons with previous methods. The performance of \textbf{Plain Model$^\dagger$} reported in \cite{liu2019large} is trained only in 30 epochs. The \textbf{OLTR}$^\dagger$ \cite{liu2019large} is trained with \textbf{Resample}\cite{shen2016relay} in default. The second block of 5 rows shows the results of our re-implement baselines. For fair comparison, we report the performance of \textbf{Plain Model} which is trained with extra 60 epochs same with \cite{liu2019large}. The last block of 4 rows present the performance of re-balancing method equipped with our method and OLTR\cite{liu2019large}.}
%\vspace{-0.8em}
%% \begin{threeparttable}
% \resizebox{0.999\textwidth}{!}{
%\begin{tabular}{l|c||c|ccc||c|ccc}
%\toprule
%\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}}  & \multicolumn{4}{c||}{\textbf{Top-1 Accuracy}} & \multicolumn{4}{c}{\textbf{Top-5 Accuracy}}\\
%\cmidrule{3-9}
%              & & \textbf{Average} & \textbf{Many-shot} & \textbf{Medium-shot} & \textbf{Few-shot} &  \textbf{Average} & \textbf{Many-shot} & \textbf{Medium-shot} & \textbf{Few-shot} \\
%\midrule
%Naive\cite{kang2019decoupling}  & R-50 & 41.6	             & 64.0               &          33.8        &  5.8  & \\
%NCM\cite{kang2019decoupling}   & R-50  & 44.3             & 53.1               &          42.3        &  26.5 & \\
%cRT\cite{kang2019decoupling}    & R-50 & 47.3             & 58.8              &    44.0   & 26.1    & \\
%$\tau$-Norm\cite{kang2019decoupling}  & R-50 & 46.7        & 56.6              &    44.2   & 27.4    & \\
%LWS\cite{kang2019decoupling}          & R-50 & 47.7        & 57.1              &    45.2   & 29.3   & \\
%Logit Adjust(Post)\cite{} & R-50 & 50.3  & - &- &-\\
%%Logit Adjust(Loss)\cite{} & R-50 & 51.1  & - &- &-\\
%\midrule
%Naive$^\dagger$   & R-50 & 45.2        &  67.4               &    38.0    & 7.5 & \\
%Cosine$^\dagger$  & R-50 & 48.4        &  68.4               &    41.8    & 15.2 & \\
%cRT$^\dagger$\cite{kang2019decoupling} & R-50 & 51.1         &    63.4    & 48.7   & 29.5    & \\
%Logit Adjust(Post)$^\dagger$\cite{} & R-50 & 50.8  & 62.8 & 48.6 & 24.9   &-\\
%
%%\textbf{DisCal-Naive}(Non-parametric) & R-50  &    \\
%\textbf{DisCal-Naive}(Learnable)      & R-50  &  51.7 & 62.3 & 48.7 & \textbf{32.1} &  \\
%\textbf{DisCal-Cosine}(Learnable)      & R-50 &  \textbf{52.8} & 65.2 & \textbf{49.8} & 28.0 & \\
%\midrule
%Naive\cite{}  & X-50 & 44.4	             & 65.9               &          37.5        &  7.7  & \\
%NCM\cite{}   & X-50  & 47.3              & 56.6               &          45.3        &  28.1 & \\
%cRT\cite{}    & X-50 & 49.6              & 61.8               &          46.2   &     27.4    & \\
%$\tau$-Norm\cite{} & X-50 & 49.4         & 59.1               &          46.9   &     30.7    & \\
%LWS                & X-50  & 49.9        & 60.2               &          47.2   &     30.3   & \\
%Deconfound\cite{}         & X-50  & 51.8        & 62.7               &          48.8  &     31.6   & \\
%\midrule
%Naive$^\dagger$   & X-50  & 46.8        &  68.1               &    40.2    & 9.3 & \\
%Cosine$^\dagger$  & X-50  & 49.2        &  68.9               &    42.8    & 15.6 & \\
%\textbf{DisCal}(Non-parametric) & X-50  &   \\
%\textbf{DisCal}(Learnable)      & X-50  &   \\
%%\midrule
%%Plain Model \cite{he2016deep}$^\dagger$    & 20.9 & 40.9 & 10.7 & 0.4 & - & - & - & - \\
%%+ Lifted Loss \cite{oh2016deep}    & 30.8 & 35.8 & 30.4 & 17.9 & - & - & - & - \\
%%+ Focal Loss\cite{lin2017focal}    & 30.5 & 36.4 & 29.9 & 16.0 & - & - & - & - \\
%%+ Range Loss\cite{zhang2017range}  & 30.7 & 35.8 & 30.3 & 17.6 & - & - & - & - \\
%%+ FSLwF\cite{gidaris2018dynamic}   & 28.4  & 40.9 & 22.1 & 15 & - & - & -  \\
%%+ Resample\cite{shen2016relay} + OLTR\cite{liu2019large}$^\dagger$   & \textbf{35.6} & 43.2 & 35.1 & 18.5 & - & - & - & - \\
%%\midrule
%\bottomrule
%\end{tabular}}
%%\end{threeparttable}
%\label{tab:classification}
%\end{table*}


\subsection{Object Detection on LVIS Dataset}



==> sections/experiments_bak_v2.tex <==

\section{Experiments}\label{sec:exp}
In this section, we conduct a series of experiments to validate the effectiveness of our method. Below we present our experimental analysis and ablation study on the image classification task in Sec. \ref{subsec:classification}, followed by our results on semantic segmentation task in Sec. \ref{subsec:seg}.  And we also evaluate our methods on object detection and instance segmentation tasks in Sec.\ref{subsec:detection}. In each task, we first introduce the implementation details of our method, and then report comparisons of quantitative results on each dataset.

\subsection{Image Classification}\label{subsec:classification}
\subsubsection{Experimental Details}
\paragraph{Datasets and Evaluation Metrics} 
To demonstrate our methods, we conduct experiments on three large-scale long-tailed datasets, including Places-LT\cite{liu2019large}, ImageNet-LT\cite{liu2019large}, and iNaturalist 2018\cite{van2018inaturalist}. Places-LT and ImageNet-LT are artificially generated by sampling a subset from their balanced versions (Places-365\cite{liu2019large} and ImageNet-2012\cite{deng2009imagenet}) following the \textit{Parento distribution}. 
%Places-LT contains images from 365 categories and the number of images per class ranges from 4980 to 5. ImageNet-LT has 1000 classes and the number of images per class ranges from 1280 to 5 images. 
iNaturalist 2018 is a real-world, naturally long-tailed dataset, consisting of samples from 8,142 species. 
We report the class-balanced average \textit{top-1} accuracy on corresponding validation/test set, and also calculate the accuracy of three disjoint subsets: \textit{many-shot classes}($>$100 training instances), \textit{medium-shot classes}(20$\sim$100 training instances) and \textit{few-shot classes}($<$20 training instances).

\paragraph{Training Configuration.}
Following \cite{kang2019decoupling}, we use PyTorch\cite{paszke2019pytorch} framework for all experiments. For ImageNet-LT, we report performance with ResNet-\{50,101,152\} and ResNeXt-\{50,101,152\} and mainly use ResNet-50 for ablation study. For iNaturalist 2018, performance is reported with ResNet-\{50,101,152\}. For Places-LT, ResNet-152 is used as backbone and we pre-train it on the full ImageNet-2012 dataset. We use the SGD optimizer with momentum 0.9, batch size 256, cosine learning rate schedule gradually decaying from 0.1 to 0 and image resolution 224$\times$224. For the representation learning stage, the backbone network are trained with 90/200 epochs. In the second distribution align stage, we restart the learning rate and train it for 10 epochs as \cite{kang2019decoupling} while keeping the backbone network and classifier fixed.

%\begin{table}[t!]
%	\centering
%	\caption{\textbf{Average accuracy on iNaturalist-2018.} Detailed comparison is reported in supplementary, and $*$ is for cosine classifier.}
%		\vspace{-0.8em}
%	\resizebox{0.49\textwidth}{!}{
%		\begin{tabular}{l|cc|cc}
%			\toprule
%				\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{90 Epoch}}         & \multicolumn{2}{c}{\textbf{200 Epoch}} \\
%				\cmidrule{2-5}
%				                                 &  \textbf{Acc@R-50}      &  \textbf{Acc@R-152}    & \textbf{Acc@R-50}         & \textbf{Acc@R-152}\\
%				\midrule
%				Baseline                            &  61.7        &  65.0    & 65.8       & 69.0\\
%				Baseline$^*$                        &  64.8        &  67.3    & 66.2       & 69.0\\
%				\midrule
%				LDAM\cite{cao2019learning} 								& 64.6         & -        & -         & -\\
%				LDAM+DRW	\cite{cao2019learning}                           & 68.0         & -        & -         & -\\
%				cRT\cite{kang2019decoupling}                              &  65.2        &  68.5    & 68.2       & 71.2\\
%				$\tau$-norm\cite{kang2019decoupling}                      &  65.6        &  68.8      & 69.3     & 72.5\\
%				LWS\cite{kang2019decoupling}                              &  65.9	    &  69.1      & 69.5     & 72.1\\
%				BBN\cite{zhou2020bbn}            &  66.3	    & -           & 69.6    & - \\
%				\midrule
%				\textbf{DisAlgin}                &  67.8   &  71.3  & \textbf{70.6}          & \textbf{74.1}  \\ % Scale=1.2
%				\textbf{DisAlgin$^*$}      &  \textbf{69.5}   &  \textbf{71.6}   & 70.2  & 72.8 \\
%%				\textbf{DisAlgin}                &  67.8\more{(+1.5)}   &  71.3\more{(+2.2)}   & 70.6\more{(+1.0)}         & 74.1\more{(+1.6)} \\ % Scale=1.2
%%				\textbf{DisAlgin$^*$}      &  69.5\more{(+3.2)}   &  71.6\more{(+2.5)}   & 70.2\more{(+0.6)} & 72.8\more{(+0.3)}\\
%			\bottomrule
%		\end{tabular}
%	}
%	\label{tab:inaturalist}
%\end{table}


\begin{table}[t!]
	\centering
	\caption{\textbf{Average accuracy on iNaturalist-2018.} Detailed comparison is reported in supplementary, and $*$ is for cosine classifier.}
		\vspace{-0.8em}
	\resizebox{0.495\textwidth}{!}{
		\begin{tabular}{l|cc|cc}
			\toprule
				\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{ResNet-50}}         & \multicolumn{2}{c}{\textbf{ResNet-152}} \\
				\cmidrule{2-5}
%				                                 &  \textbf{Acc@90E}      &  \textbf{Acc@200E}    & \textbf{Acc@90E}         & \textbf{Acc@200E}\\
				                                 &  \textbf{90 Epoch}      &  \textbf{200 Epoch}    & \textbf{90 Epoch}         & \textbf{200 Epoch}\\
				\midrule
				Baseline                            &  61.7            & 65.8  &  65.0     & 69.0\\
				Baseline$^*$                        &  64.8          & 66.2  &  67.3       & 69.0\\
				\midrule
				LDAM\cite{cao2019learning} 								& 64.6         & -        & -         & -\\
				LDAM+DRW	\cite{cao2019learning}                           & 68.0         & -        & -         & -\\
				cRT\cite{kang2019decoupling}                              &  65.2        & 68.2  &  68.5         & 71.2\\
				$\tau$-norm\cite{kang2019decoupling}                      &  65.6          & 69.3 &  68.8        & 72.5\\
				LWS\cite{kang2019decoupling}                              &  65.9	     & 69.5 &  69.1         & 72.1\\
				BBN\cite{zhou2020bbn}            &  66.3	   & 69.6 & -               & - \\
				\midrule
				\textbf{DisAlgin}                &  67.8    & \textbf{70.6} &  71.3          & \textbf{74.1}  \\ % Scale=1.2
				\textbf{DisAlgin$^*$}      &  \textbf{69.5}   & 70.2   &  \textbf{71.6}  & 72.8 \\
%				\textbf{DisAlgin}                &  67.8\more{(+1.5)}   &  71.3\more{(+2.2)}   & 70.6\more{(+1.0)}         & 74.1\more{(+1.6)} \\ % Scale=1.2
%				\textbf{DisAlgin$^*$}      &  69.5\more{(+3.2)}   &  71.6\more{(+2.5)}   & 70.2\more{(+0.6)} & 72.8\more{(+0.3)}\\
			\bottomrule
		\end{tabular}
	}
	\label{tab:inaturalist}
\end{table}


\subsubsection{Comparison with the state-of-the-art methods}
\paragraph{ImageNet-LT.} We present the quantitive results for ImageNet-LT in Table \ref{tab:imagenet_lt}. Compared to the state-of-the-art methods, our approach can achieve \textbf{52.9\%} with a large margin performance gain at \textbf{2.6} based on ResNet-50 backbone and and \textbf{53.4\%} with a margin of \textbf{1.6} based on ResNeXt-50. 
%Moreover, we find  training only for 90 epochs gives sub-optimal representations, and it could be further improved by training with 200 epochs like iNaturalist, which results in a higher performance(\textbf{53.7\%} with ResNet-50 and \textbf{54.4\%} with ResNeXt-50) with our proposed \textbf{DisAlign}.


\begin{table}[t!]
	\centering
	\caption{\textbf{Results on Place365-LT.} More results of different backbones are reported in supplementary, and $*$ is for cosine classifier. }
\vspace{-0.8em}
	\resizebox{0.44\textwidth}{!}{
		\begin{tabular}{l|l|ccc}
			\toprule
				\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{ResNet-152}} \\
				\cmidrule{2-5}
				                                 &  \textbf{Average}                  &  \textbf{Many}                      & \textbf{Medium}                      &  \textbf{Few}\\
				\midrule
				Focal Loss\cite{liu2019large}                &  34.6                     & 41.1                       &    34.8                     &  22.4\\
				Range Loss\cite{liu2019large} &  35.1                     & 41.1                       &    35.4                     &  23.2\\
				OLTR\cite{liu2019large}       &  35.9                     & 44.7                       &    37.0                     &  25.3\\					
				Baseline 						     &  30.2                     & 46.3                       &    27.7                     &  9.5\\
%				Baseline$^*$\\
				\midrule
				NCM & 36.4                     & 40.4       & 37.1 & 27.3\\
				cRT & 36.7                     & 42.0       & 37.6 & 24.9\\
				LWS & 37.6                     & 40.6       & 39.1 & 28.6\\
				$\tau$-norm          &  37.9   & 37.8       & 40.7 & 31.8\\
				\midrule
				\textbf{DisAlgin}                & \textbf{39.3} & 40.4 & 42.4 & 30.1 \\
%				\textbf{DisAlgin$^*$}      & 00.0\more{(+0.0)} \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:places}
\end{table}


\paragraph{iNaturalist and Places-LT.} To further demonstrate our method, we conduct experiments on two extra large-scale long-tail benchmark and report the performance in Table \ref{tab:inaturalist} and Table \ref{tab:places}. For iNaturalist, DisAlign with cosine classifier achieve \textbf{69.5\%} with a large margin at \textbf{1.5} on ResNet-50(90 epoch). The performance could be improved sustainedly with larger backbone and more training epochs. For Places-LT, we follow \cite{kang2019decoupling} and compare our method with recent works based on ResNet-152, which achieve \textbf{39.3\%} with a large margin at \textbf{1.4}. We also reported the detailed performance of these two datasets with ResNet-\{50,101,152\} in supplementary materials. %Results of these two datasets demonstrate the effectiveness of our method.

\begin{table}[t!]
	\centering
	\caption{\textbf{Ablation study of DisAlign.} \textbf{GR} means the generalized reweight strategy.  \textbf{MT} means the learnable magnitude parameter (1+$\sigma(\mathbf{x})\alpha$) and \textbf{MG} is the learnable margin parameter  $\sigma(\mathbf{x})\beta$.}
    \vspace{-0.8em}
	\resizebox{0.45\textwidth}{!}{
		\begin{tabular}{c|l|l|c|ccc}
			\toprule
%				\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{90 Epoch} & \multicolumn{2}{c}{200 Epoch} \\
%				\cmidrule{2-5}
%				                                 &  Res50                    &  Res152                     & Res50                      & Res152\\
%				ID & Magnitude $\alpha$            &  Margin $\beta $                  &  Average                   & Many              & Medium         & Few \\
				\textbf{GR}  & \textbf{MT}         & \textbf{MG}                &  \textbf{Average}                   & \textbf{Many}              & \textbf{Medium}         & \textbf{Few} \\
				\midrule
				\xmark & \xmark                           & \xmark &   41.6	           & 64.0           &    33.8         &  5.8\\
				\cmark & \cmark                           & \xmark &\\
				\cmark & \xmark                           & \cmark &\\
				\cmark & \cmark                           & \cmark & 51.3 & 59.9& 49.9 &31.8\\
%				\midrule
%				\textbf{DisAlgin}                &  61.7\colorpm{$\pm0.00$}  &  65.0\colorpm{$\pm0.00$}    & 65.8\colorpm{$\pm0.00$}    & 69.0\colorpm{$\pm0.00$} \\
%				\textbf{DisAlgin$^\dagger$}                &  61.7\colorpm{$\pm0.00$}  &  65.0\colorpm{$\pm0.00$}    & 65.8\colorpm{$\pm0.00$}    & 69.0\colorpm{$\pm0.00$} \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:model_ablation}
\end{table}
%
%\begin{table*}[h!]
%\centering
%\caption{\textbf{Performance of semantic segmentation  on ADE-20K:} All baseline models are trained with an image size of 512$\times$512 and 160K iteration in total. B means the type of backbone network(denoted as R-50, R-101, S-101 for ResNet-50, ResNet-101 and ResNeSt-101)}
%\vspace{-0.8em}
%\resizebox{0.999\textwidth}{!}{
%\begin{tabular}{l|c||l|lll||l|lll}
%\toprule
%\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{B}} & \multicolumn{4}{c||}{\textbf{Mean IoU}} & \multicolumn{4}{c}{\textbf{Mean Accuracy}}\\
%\cmidrule{3-10}
%              & & \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} &  \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} \\
%\midrule
%%% FCN with Res-50
%FCN\cite{kang2019decoupling}  & \multirow{2}{*}{R-50}    & 38.1  &  64.6   &  40.0   & 29.6 
%															  & 46.3  &  78.6   &  49.3   & 35.4 \\
%\textbf{FCN+DisAlign}         &                       & 40.1\more{(+2.0)}  & 65.0\more{(+0.4)}  & 42.8\more{(+2.6)} & 31.3\more{(+2.5)}   
%															  & 51.4\more{(+5.1)}  & 78.6\small{(+0.0)} & 56.1\more{(+5.8)} & 40.6\more{(+5.2)}\\
%\midrule
%%% FCN with Res-101
%FCN\cite{kang2019decoupling}  &  \multirow{2}{*}{R-101}     &  41.4  &   67.0  &  43.3   & 33.2 
%																   &  50.2  &   80.6  &  52.9   & 40.1 \\
%\textbf{FCN+DisAlign}         &                             &  43.7\more{(+2.3)}  & 67.4\more{(+0.4)}  & 46.1\more{(+2.8)} & 35.7\more{(+2.5)}   
%														           &  55.9\more{(+5.7)}  & 80.6\small{(+0.0)} & 59.7\more{(+4.8)} & 46.4\more{(+6.3)}  \\
%\midrule
%%% FCN with Res-101
%FCN\cite{kang2019decoupling}  &  \multirow{2}{*}{S-101}          & 46.2  & 67.6   & 48.0  & 39.1 
%																	  & 57.3  & 79.4   & 61.7  & 48.2   \\
%\textbf{FCN+DisAlign}         &                              & 46.9\more{(+0.7)}  & 67.7\more{(+0.1)}  & 48.2\more{(+0.2)}  & 40.3\more{(+1.2)}
%																      & 60.1\more{(+2.8)} &  79.7\more{(+0.3)}  & 64.2\more{(+2.5)}  & 51.9\more{(+3.7)} \\
%\midrule
%\midrule
%%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} & \multirow{2}{*}{R-50}   &  44.9  &  67.7  &   48.3  &   36.4 
%																		  &  55.0  &  80.1  &   60.8  &   44.1 \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                        &  45.7\more{(+0.8)} & 67.7\small{(+0.0)} & 48.6\more{(+0.3)} & 37.8\more{(+1.4)}
%																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
%\midrule
%%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{2}{*}{R-101}  &  46.4 & 68.7  & 49.0 & 38.4 & 56.7 & 80.9 & 61.5 & 47.7 \\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                        &  47.1\more{(+0.7)} & 68.7\small{(+0.0)} & 49.4\more{(+0.4)} & 39.6\more{(+1.2)}
%																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
%\midrule
%%% DeepLabV3 with Res-101
%DeepLabV3$^{+}$\cite{kang2019decoupling} &\multirow{2}{*}{S-101}  &  47.3 & 69.0 & 49.7 & 39.7
%																	      &  58.1 & 80.8 & 63.4 & 48.2\\
%\textbf{DeepLabV3$^{+}$+DisAlign}        &                       &  47.8\more{(+0.5)} & 68.9\small{(-0.1)} & 49.8\more{(+0.1)} & 40.7\more{(+1.0)} 
%																		  &  60.1\more{(+2.0)} & 81.0\more{(+0.2)}  & 65.5\more{(+2.1)} & 52.0\more{(+1.8)}\\
%\midrule
%\bottomrule
%\end{tabular}}
%\label{tab:segmentation}
%\end{table*}

\begin{table*}[h!]
\centering
\caption{\textbf{Performance of semantic segmentation  on ADE-20K:} All baseline models are trained with an image size of 512$\times$512 and 160K iteration in total. B means the type of backbone network(denoted as R-50, R-101, S-101 for ResNet-50, ResNet-101 and ResNeSt-101)}
\vspace{-0.8em}
\resizebox{0.999\textwidth}{!}{
\begin{tabular}{l|l|c||l|lll||l|lll}
\toprule
\multirow{2}{*}{\textbf{Framework}} &\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{B}} & \multicolumn{4}{c||}{\textbf{Mean IoU}} & \multicolumn{4}{c}{\textbf{Mean Accuracy}}\\
\cmidrule{4-11}
       &       & & \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} &  \textbf{Average} & \textbf{Head} & \textbf{Body} & \textbf{Tail} \\
\midrule
%% FCN with Res-50
\multirow{6}{*}{FCN\cite{shelhamer2017fully}} & Baseline & \multirow{2}{*}{R-50}    & 38.1  &  64.6   &  40.0   & 29.6 
															  & 46.3  &  78.6   &  49.3   & 35.4 \\
& \textbf{DisAlign}         &                       & 40.1\more{(+2.0)}  & 65.0\more{(+0.4)}  & 42.8\more{(+2.6)} & 31.3\more{(+2.5)}   
															  & 51.4\more{(+5.1)}  & 78.6\small{(+0.0)} & 56.1\more{(+5.8)} & 40.6\more{(+5.2)}\\
\cmidrule{2-11}
%% FCN with Res-101
& Baseline &  \multirow{2}{*}{R-101}     &  41.4  &   67.0  &  43.3   & 33.2 
																   &  50.2  &   80.6  &  52.9   & 40.1 \\
&\textbf{DisAlign}         &                             &  43.7\more{(+2.3)}  & 67.4\more{(+0.4)}  & 46.1\more{(+2.8)} & 35.7\more{(+2.5)}   
														           &  55.9\more{(+5.7)}  & 80.6\small{(+0.0)} & 59.7\more{(+4.8)} & 46.4\more{(+6.3)}  \\
\cmidrule{2-11}
%% FCN with Res-101
&Baseline  &  \multirow{2}{*}{S-101}          & 46.2  & 67.6   & 48.0  & 39.1 
																	  & 57.3  & 79.4   & 61.7  & 48.2   \\
&\textbf{DisAlign}         &                              & 46.9\more{(+0.7)}  & 67.7\more{(+0.1)}  & 48.2\more{(+0.2)}  & 40.3\more{(+1.2)}
																      & 60.1\more{(+2.8)} &  79.7\more{(+0.3)}  & 64.2\more{(+2.5)}  & 51.9\more{(+3.7)} \\
\midrule
\midrule
%% DeepLabV3 with Res-101
\multirow{6}{*}{DeepLabV3$^{+}$\cite{deeplabv3plus2018}} & Baseline & \multirow{2}{*}{R-50}   &  44.9  &  67.7  &   48.3  &   36.4 
																		  &  55.0  &  80.1  &   60.8  &   44.1 \\
&\textbf{DisAlign}        &                        &  45.7\more{(+0.8)} & 67.7\small{(+0.0)} & 48.6\more{(+0.3)} & 37.8\more{(+1.4)}
																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
\cmidrule{2-11}
%% DeepLabV3 with Res-101
& Baseline &\multirow{2}{*}{R-101}  &  46.4 & 68.7  & 49.0 & 38.4 & 56.7 & 80.9 & 61.5 & 47.7 \\
&\textbf{DisAlign}        &                        &  47.1\more{(+0.7)} & 68.7\small{(+0.0)} & 49.4\more{(+0.4)} & 39.6\more{(+1.2)}
																          &  59.5\more{(+2.8)} & 81.4\more{(+0.5)} & 64.2\more{(+2.7)} & 50.3\more{(+2.6)} \\
\cmidrule{2-11}
%% DeepLabV3 with Res-101
&  Baseline &\multirow{2}{*}{S-101}  &  47.3 & 69.0 & 49.7 & 39.7
																	      &  58.1 & 80.8 & 63.4 & 48.2\\
&\textbf{DisAlign}        &                       &  47.8\more{(+0.5)} & 68.9\small{(-0.1)} & 49.8\more{(+0.1)} & 40.7\more{(+1.0)} 
																		  &  60.1\more{(+2.0)} & 81.0\more{(+0.2)}  & 65.5\more{(+2.1)} & 52.0\more{(+1.8)}\\
\midrule
\bottomrule
\end{tabular}}
\label{tab:segmentation}
\end{table*}





\subsubsection{Ablation Study}
\paragraph{Different Backbone:} We validate our method on different backbone networks, ranging from ResNet-\{50,101,152\} to ResNeXt-\{50, 101, 152\}, reported in Figure \ref{fig:backbones}. It's worth noting that even when adopting stronger backbones, the gain of DisAlign compared to the state-of-the-art methods is still significant, which demonstrates that our DisAlign is complementary to the capacity of current models. With DisAlign, we can achieve \textbf{54.9} with ResNet-152, and \textbf{55.0} with ResNeXt-152.
\begin{figure}
    \centering
    \includegraphics[width=0.999\linewidth]{figs/backbone_ablation}
        \vspace{-2.8em}
    \caption{\textbf{Performance of DisAlign with different backbone on ImageNet-LT.} Detailed results will be reported in supplementary material.}
    \label{fig:backbones}
\end{figure}
\begin{figure}
    \centering

    \includegraphics[width=0.999\linewidth]{figs/ablation_exp_scale}
        \vspace{-2.8em}
    \caption{\textbf{Effects of the different generalized reweight scale.} Performance are reported on ImageNet-LT val split.}
    \label{fig:exp_scale_ablation}
\end{figure}

\paragraph{Model Components:}
\rev{(need to be revised)}We conduct a series of ablation studies to evaluate the importance of each component used in our DisAlign method. Table \ref{tab:model_ablation} summarize the results of our ablation experiments, in which we compare our full model with several partial model settings. First, we can see the learnable magnitude could achieve a significant improvement compared with baseline, which can also be considered as a generalized version of $\tau$-normalized\cite{kang2019decoupling} and LWS\cite{kang2019decoupling}. Second, we find the learnable margin could achieve \textbf{0.0}, which is a generalized version of Logit Adjustment\cite{menon2020long} and Deconfound\cite{tang2020long}.

\paragraph{Generalized Reweight Scale}
We also investigate the influence of the generalized reweight scale on the validation set of ImageNet-LT and plot the accuracy-scale curve in Figure \ref{fig:exp_scale_ablation}. It is evident that adjusting generalized reweight is able to achieve significant performance improvement. Moreover, we find $\epsilon>1$ could outperform the class-balanced rewegiht($\epsilon=1$), which indicates that generalized reweight more flexible to adaptive for different imbalanced situation by choosing a approximate scale.% compared with the hand-craft reweight strategy.

\subsection{Semantic Semgnetaion on ADE20k Dataset}\label{subsec:seg}
Similar with image classification, the large-scale semantic segmentation task still suffers from the long-tail data distribution. To further validate effectiveness of our method, we also apply DisAlign on large-scale semantic segmentation benchmark: ADE20k. 




\begin{table*}
\caption{\textbf{Comparison with the-state-of-art on LVIS with Mask-R-CNN-FPN(ResNet-50 backbone).} All experiments results are evaluated on the LVIS v0.5 validation set with the score threshold at 0.0001. ($*$ means the cosine classifier is used for bounding box classification.)}
\label{tab:lvis_sota}
\vspace{-0.8em}
\centering
    \resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|l|c|ccc|c|ccc}
\toprule
  \multirow{2}{*}{\textbf{Pre-Train}}& \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{Box AP}} & \multicolumn{4}{c}{\textbf{Mask AP}} \\
  \cmidrule{3-10}
  &  & $\text{AP}_{bbox}$ & $\text{AP}_{bbox}^r$ & $\text{AP}_{bbox}^c$ & $\text{AP}_{bbox}^f$ & $\text{AP}_{mask}$& $\text{AP}_{mask}^r$ & $\text{AP}_{mask}^c$ & $\text{AP}_{mask}^f$ \\
\midrule
 \multirow{8}{*}{ImageNet}	 & Baseline 	                & 20.8  &  3.3   &  19.5  & 29.4     & 21.2 &   3.7  & 21.6 & 28.4  \\
          & Baseline$^{*}$ 	            &                    22.8  &  10.2  &  21.1  & 30.1     & 23.8 &   11.5 & 23.7 & 28.9 \\
          &Focal Loss\cite{lin2017focal}                                      & 21.9  & -      & -      & -        & 21.0 & 9.3 & 21.0 & 25.8 \\
          &SimCal\cite{wang2020devil}				                & 22.6  &  13.7  &  20.6  & 28.7     & 23.4 &   \textbf{16.4} & 22.5 & 27.2 \\ % Checked
          &RFS\cite{gupta2019lvis}				                  & 23.6  &	12.8  &  22.3  & 29.4     & 24.3 &   14.6 & 24.0 & 28.5\\
          &EQL\cite{tan2020equalization}			              & 23.3  &  -     &  -     & -        & 22.8 &   11.3 & 24.7 & 25.1 \\
\cmidrule{2-10}
         &  \textbf{DisAlign}                                 & 23.9   & 7.5    & 25.0   & 29.1     & 24.3 & 8.5 & 26.3 & 28.1\\
          & \textbf{DisAlign$^*$}                          & \textbf{25.6} &  \textbf{13.7} & \textbf{25.6} & \textbf{30.5} & \textbf{26.3} & 14.9 & \textbf{27.6} &  \textbf{29.2} \\
%\cmidrule{1-10}
\midrule
%\midrule
 \multirow{6}{*}{COCO} 	&  Baseline			  &  22.8 &  2.6  &  21.8 & 32.0     & 23.9 & 2.8 & 23.4 & 30.5  \\
   & Baseline$^*$ 	  &                        25.0 &  10.2  & 23.9 & 32.3     & 25.3 & 11.0 & 25.5 & 30.7 \\
%\cmidrule{1-2}\cmidrule{4-10}
%& RFS\cite{gupta2019lvis}  &   &    & \\
%EQL\cite{gupta2019lvis}  & & 	& - & - &  - & - & 24.4 & 14.5& 24.3 & 28.4 \\
%Forest R-CNN	 		 & &   								& 25.9 & 16.9 & 26.1 & 29.2       & 25.6 & 18.3 & 26.4 & 27.6\\  
  &  GroupSoftmax\cite{li2020overcoming}       & 25.8 & 15.0 & 25.5 & 30.4       & 26.3 & \textbf{18.0} & 26.9 & 28.7 \\
%SimCal\cite{}            & &                                  & 22.6 & 13.7   & 20.6 & 28.7     & 23.4 & 16.4 & 22.5 & 27.2 \\
\cmidrule{2-10}
  & \textbf{DisAlign}            &    25.5 & 8.2 & 26.3 & 32.4 & 25.7 & 9.4 & 27.6 & 29.7 \\
  & \textbf{DisAlign$^*$}          &	   \textbf{27.6} & 14.8   & \textbf{27.9} & \textbf{32.4}    & \textbf{27.9} & 16.2 & \textbf{29.3} & \textbf{30.8}\\
\bottomrule
\end{tabular}}
\end{table*}

\subsubsection{Dataset and Implementation Details}
\paragraph{Dataset.} ADE20K dataset is a scene parsing benchmark, which contains 150 stuff/object categories. The dataset includes 20K/2K/3K images for training, validation and testing. Compared with the image classification\cite{liu2019large}, the imbalance of ADE20K is more serve than the image classification, which has a imbalance ratio of \textbf{788}(Max/Min). Follow the similar protocol in image classification, we divide the 150 categories into 3 groups according to ratio of pixel number over whole dataset. Specifically, three disjoint subsets are: \textit{head classes}(classes each with a ratio over 1.0\%), \textit{body classes}(classes each with a ratio ranging from 0.1\% to 1\%) and \textit{tail classes}(classes under a ratio of 0.1\%), complete list of the split is reported in supplementary material.

\paragraph{Implementation Details.} We implement our method based on MMSegmentation toolkit\cite{mmsegmentation}. In the representation learning training phase, we set the learning rate to 0.01 initially, which gradually decreases to 0 by following the 'poly' strategy as \cite{zhang2018context}. The images are cropped to $512\times 512$ and augmented with randomly scaling(from 0.5 to 2.0) and flipping. ResNet-50, ResNet-101 and ResNeSt-101\cite{} are used as the backbone. For the evaluation metric, we use the mean intersection of union(mIoU) and mean pixel accuracy(mAcc). All models are trained with 160k iterations with a batch size of 32 based on 8 V100 GPUs. In the DisAlign stage, we follow the similar protocol as the stage-1 and only training the model with 8k iterations.
% All experiments are conducted on 8 Titan-Xp GPUs with batch size 16. 
% Our method achieves 42.64\% mIoU with ResNet-50 backbone, outperforms the recent method EncNet(\cite{zhang2018context}) by 1.5\%. We also validate our method on the online test benchmark by fine-tuning the model on \text{trainval} set for another 40 epochs with learning rate 0.0005, and our method outperforms other methods with a final score of 0.5615, shown in Tab.\ref{tab:seg_speed}.
\subsubsection{Quantitative Results}
We evaluate our methods with two state-of-the-art segmentation models(FCN\cite{shelhamer2017fully} and DeepLabV3+\cite{deeplabv3plus2018})based on different backbone networks, ranging from ResNet-50, ResNet-101 to the latest ResNeSt-101, and report the performance in Tab.\ref{tab:segmentation}. 

Our method can achieve \textbf{2.0} and \textbf{2.3} mIoU improvement on FCN-8s with ResNet-50 and ResNet-101, respectively. The performance on the body and tail are improved significantly. Moreover, our method can outperform the baseline with large margin at \textbf{5.7} on mean accuracy  with ResNet-101 backbone. Even with a stronger backbone: \textbf{ResNeSt-101}, our method can also have a \textbf{0.7} mIoU and \textbf{2.8} mean accuracy improvement, where the tail categories have a performance gain of \textbf{1.2} mIoU and \textbf{3.7} mean accuracy.

We further validate our method use DeepLabV3+, which is a more powerful semantic segmentation model. Our DisAlign can improve the DeepLabV3+ to \textbf{47.8} with a margin at \textbf{0.5} based on ResNeSt-101, which achieves the state-of-the-art in ADE20k dataset.

\subsection{Object Detection on LVIS Dataset}\label{subsec:detection}

\subsubsection{Experimental Configuration}
\paragraph{Dataset.}
 LVIS\cite{gupta2019lvis} dataset is a benchmark dataset for research on large vocabulary object detection and instance segmentation, which contains 56K images over 1230 categories for training, 5K images for validation. This challenging dataset is an appropriate benchmark to study the large-scale long-tail problem, where the categories can be binned into three types similar with ImageNet-LT: \textit{rare}(1-10 training images), \textit{common}(11-100 training images) and \textit{frequent}($>100$ training images).  
 \paragraph{Evaluation Protocol.}
 We evaluate our method on LVIS for object detection and instance segmentation. For evaluation, we use a COCO-style average precision(AP) metric that averages over categories and different box/mask intersection over union(IoU) threshold\cite{lin2014microsoft}. All standard LVIS evaluation metrics including $\text{AP}, \text{AP}^{r}, \text{AP}^{c}, \text{AP}^{f} $ for box bounding boxes and segmentation masks. Subscripts ‘r’, ‘c’, and ‘f’ refer to rare, common and frequent category subsets.
 
%has a long tail distribution of the training samples of each category. Thus it is
%LVIS dataset is a benchmark dataset for research on large vocabulary instance segmentation. This challenging dataset contains 56K images over 1230 categories for training, 5K for validation. LVIS naturally has a long tail of categories with few training samples due to the Zipfian distribution of categories in natural images. LVIS is an appropriate benchmark to study the large-scale long-tail problem, where the categories can be binned into three types similar with ImageNet-LT: \textit{rare}(1-10), \textit{common}(11-100 images) and \textit{frequent}($>100$ images).

\paragraph{Implementation Details.}
We train our models for object detection and instance segmentation based on Detecron2\cite{wu2019detectron2}, which is implemented in PyTorch. Unless specified, we use the ResNet backbone(pre-trained on ImageNet) with FPN\cite{lin2017feature}. 
Following the training procedure in \cite{gupta2019lvis}, we resize the images so that the shorter side is 800 pixels. All baseline experiments are conducted on 8 GPUs with 2 images per GPU for 90K iterations, with a learning rate of 0.02 which is decreased by 10 at the 60K and 80K iteration. We use SGD with a weight decay of 0.0001 and momentum of 0.9. Scale jitter is applied for all experiments in default same with \cite{gupta2019lvis}. For the DisAlign, we freeze all network parameters and learn the magnitude and margin for extra 9K iterations with a learning rate of 0.02. Generalized reweight scale $\epsilon$ is set to 0.8 for all experiments.

%\paragraph{Evaluation Protocol.}

\subsubsection{Quantitive Results and Ablation Study}
We first compare our method with recent works and report results in Table.\ref{tab:lvis_sota}. We find DisAlign can achieve \textbf{25.6} $\text{AP}_{bbox}$, and \textbf{26.3} $\text{AP}_{mask}$ with Mask R-CNN FPN(ResNet-50) based on the ImageNet pre-trained model, and achieve \textbf{27.6} $\text{AP}_{bbox}$ and \textbf{27.9} $\text{AP}_{mask}$ based on COCO pre-trained model. Our method can maintain the performance of the frequent(also called \textit{head}) categories, and achieve significant improvement on common(also called \textit{body}) and rare(also called \textit{tail}) categories.

We also report performance with more power framework(\textit{e.g.} Cascade R-CNN) and more stronger backbones(\textit{e.g.} ResNet-\{50,101\} and ResNeXt-101) in Table.\ref{tab:lvis_ablation} It is worth noting that even when adopting stronger backbones or framework, the gain of DisAlign network compared to the baseline is still significant, which demonstrates that our method is complementary to the capacity of the current baseline models. 
 
\begin{table}
\centering
\caption{\textbf{Object detection and instance segmentation performance on LVIS v0.5 dataset.} The results are reported based on the Detectron2\cite{wu2019detectron2} framework. The detailed comparison with the-state-of-art works is reported in Supplementary.}
\vspace{-0.8em}
\resizebox{0.485\textwidth}{!}{
\begin{tabular}{c|l|ll|ll}
\toprule
  \multirow{2}{*}{\textbf{B}} & \multirow{2}{*}{\textbf{Method}}     & \multicolumn{2}{c|}{\textbf{Mask R-CNN}} &\multicolumn{2}{c}{\textbf{Cascade R-CNN}}  \\
 \cmidrule{3-6}
  &  &$\text{AP}_{bbox}$ & $\text{AP}_{mask}$   & $\text{AP}_{bbox}$ & $\text{AP}_{mask}$   \\
\midrule
\multirow{4}{*}{R-50 } & Baseline        & 20.8                 & 21.2               &  25.2            & 23.0         \\
& \textbf{DisAlgin}                   & 23.9\more{(+3.1)}   & 24.2\more{(+3.0)}   & 28.7\more{(+3.5)} & 26.1\more{(+3.1)}      \\
 \cmidrule{2-6}
& Baseline$^{*}$                          & 22.8                & 23.8                &  28.8              & 26.2         \\
& \textbf{DisAlgin$^{*}$}             & 25.6\more{(+2.8)}   & 26.2\more{(+2.4)}   &  32.2\more{(+3.4)} & 29.4\more{(+3.2)} \\
\midrule
\multirow{4}{*}{R-101 } & Baseline       & 22.2                & 22.6                &  26.1              & 24.0         \\
& \textbf{DisAlgin}                   & 25.6\more{(+3.4)}   & 25.8\more{(+3.2)}   &  29.7\more{(+3.6)} & 27.3\more{(+3.3)}\\
 \cmidrule{2-6}
& Baseline$^{*}$                          & 24.5                & 25.1                &  30.4              & 28.1        \\
& \textbf{DisAlgin$^{*}$}             & 27.5\more{(+3.0)}   & 28.2\more{(+3.1)}       &  33.7\more{(+3.3)} & 30.9\more{(+2.8)}\\
\midrule
\multirow{4}{*}{X-101 } & Baseline     & 24.5                & 25.0               &  28.4              & 26.1         \\
 & \textbf{DisAlgin}                  & 26.8\more{(+2.3)}   & 27.4\more{(+2.4)}   &  31.3\more{(+2.9)} & 28.7\more{(+2.6)} \\
 \cmidrule{2-6}
& Baseline$^{*}$                      & 26.9                & 27.7                &  31.3              & 28.7\\
& \textbf{DisAlgin$^{*}$}             & 29.5\more{(+2.6)}   & 30.0\more{(+2.3)}   &  34.7\more{(+3.3)} & 31.8\more{(+3.1)} \\
\bottomrule
\end{tabular}}
\label{tab:lvis_ablation}
\end{table}


==> sections/method_bak.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/empirical_analysis}
%	\vspace{-0.4cm}    
	\vspace{-0.8em}
    \caption{\textbf{Empirical analysis of the performance bottleneck.} \textit{Left}: Empirical classifier bound of feature extractor learned with different sampling strategy. \textit{Right}: Comparison of previous work and empirical classification bound based on instance-balanced feature extractor. \textbf{Cls-Bound} means the classifier is re-trained on the full ImageNet set(w/o. ImageNet-LT val set). \textbf{IB} is instance balanced sampling, \textbf{CB} is class-balanced sampling and \textbf{SR} is the square-root sampling.}
    \label{fig:upperbound}
\end{figure}


\section{Our Approach}
Our goal is to improve the large-scale long-tail recognition system by \textit{calibrating the mismatched distributions} of the training set and the evaluation metrics\rev{(evaluation metric or evaluation set? eval set for segmentation is also imbalanced)}. To this end, we review the current two-stage methods and unify them into a generic framework from the distribution mismatch perspective. Based on this, we develop a simple and effective distribution alignment method to improve classification on several large-scale long-tail visual recognition tasks.

Below we start with a brief introduction to the long-tail recognition task and the empirical study of the upper-bound in Sec.\ref{subsec:overview}, followed by our proposed distribution alignment strategy in Sec.\ref{subsec:alignment}. We then present the comparison and analysis of the previous methods from the distribution mismatch perspective in Sec.\ref{subsec:distribution_mismatch}. Finally, we describe the learning and inference process of our approach in Sec.\ref{subsec:learning_inference}.

\subsection{Preliminary}\label{subsec:overview}

In this subsection, we will first present the problem setting of long-tail recognition in mathematics. Then an empirical analysis of this task is detailed to motivate our proposed methods.

\paragraph{Problem Definition}

Given an input data $\mathbf{I}$, task of long-tail classification is targeted to predict the category of this input correctly even the training data is extremely imbalanced. The input could be instantiated as \textit{one pixel} for semantic segmentation, \textit{one instance} for object detection and \textit{one image} for image classification. 

The model is learned on the \textbf{imbalanced} dataset $\mathcal{D}_{train}$ and evaluated on the dataset $\mathcal{D}_{eval}$ with the \textbf{balanced metrics}(e.g. mean accuracy, mean IoU etc.). $\mathcal{D}_{train}$ and $\mathcal{D}_{eval}$ share the same category space $\mathcal{C}=\{c_1,\cdots,c_K\}$, where $K$ is the number of categories in one dataset.
Typically, we can formulate the model $\mathcal{M}$ with two main components: feature extractor network $f(\cdot)$ and the linear classifier head $h(\cdot)$, where $\mathcal{M}=\{f(\cdot),h(\cdot)\}$. The feature representation of $I$ is extracted with $f$ as:
\begin{align}
	\mathbf{x} &= f(\mathbf{I}, \theta_{f})\in\mathbb{R}^{d}
\end{align}
The class prediction score for input $\mathbf{I}$ is generated as:
\begin{align}
	\mathbf{z}=h(\mathbf{x},\theta_{h})\in\mathbb{R}^K
\end{align}
where $\theta_{f}$ and $\theta_{h}$ are the parameter of $f(\cdot)$ and $h(\cdot)$, respectively. And $\mathbf{z}=\{z_1,\cdots,z_K\}$ is the classification logit, the label is predicted by using the index of the $\arg\max{(\mathbf{z})}$. In this work, we instantiate the $h$ as dot-product classifier or cosine similarity classifier, as:

\begin{align}
%\setlength{\abovedisplayskip}{1pt}
%\setlength{\belowdisplayskip}{1pt}
	\text{Dot-Product}:\quad &z_j=\mathbf{w}_j^\intercal\mathbf{x}\\
	\text{Cosine Similarity}:\quad &z_j=s\cdot\frac{\mathbf{w}_j^\intercal\mathbf{x}}{||\mathbf{w}_j||||\mathbf{x}||}
\end{align}
where $\mathbf{w}_j\in\mathbb{R}^d$ is the parameter of $j$-th class and the $s$ is the scale factor introduced in \cite{qi2018low}(could be learnable parameter or constant hyper-parameter).

\paragraph{Empirical Analysis of the Performance Bottleneck}

The previous methods typically improve long-tail recognition system either from the representation(feature extractor $f$) or the decision boundary(linear classifier $h$).
 Specifically, many re-balanced strategies try to improve the $f$ and $h$ both in one-stage learning. 
 Recently, the two-stage learning strategy has demonstrate in many long-tail recognition task, in which the $f$ and $h$ are learned sequentially. 

To investigate the bottleneck of these methods, we conduct comprehensive experiments to analysis the empirical upper-bound. As we are able to access the balanced full-set of ImageNet dataset, all analysis experiments are conducted on the ImageNet-LT\cite{liu2019large} dataset. First, the $f$ is learned on the \textbf{imbalanced} $\mathcal{D}_{train}$(ImageNet-LT train set) with different re-balancing strategies. Then the $h$ for all methods is optimized on the \textbf{balanced} ImageNet train set(exclude ImageNet-LT val set) without any re-balance strategy. 

As shown in Figure \ref{fig:upperbound}, the upper-bound classifiers are learned on the balanced full set, which also indicate how discriminative(linear separability in $\mathbb{R}^d$) of the feature representation of each method. Compared with empirical upper-bound of different re-balancing solutions, we can easily found:
\vspace{-0.5em}
\begin{itemize}
	\item \textit{the instance-balanced sampling can provide the sufficient discriminative representation than other re-balance strategies},
\end{itemize} 
\vspace{-0.5em}
which is consistent with conclusion of \cite{kang2019decoupling}. 
Furthermore, for the instance-balanced methods, there still exists \textit{a large margin of performance gap} between the empirical upper-bound and the state-of-the-art methods, which means:
\vspace{-0.5em}
\begin{itemize}
	 \item \textit{the unfaithful decision boundary is the bottleneck of the current long-tail recognition system}
\end{itemize}
\vspace{-0.5em}
Addressing this issue is expected to effectively improve long-tail recognition tasks.

%A widely used pipeline, instance-balanced feature learning with classifier re-training framework is adopted in many recent works.




\subsection{Distribution Alignment}\label{subsec:alignment}
To tackle the aforementioned issue, we now introduce a \textit{unified} distribution alignment strategy to calibrate the classifier output via matching it to a reference distribution of classes that favors the balanced prediction.
\subsubsection{Principle of Distribution Alignment\rev{(need to be revised)}}


% Long-tail Feature Extractor, Balanced Classifier
%As discussed before, the instance-balanced learning strategy is able to provide sufficient discriminative representation, the main bottleneck of the system is the decision boundary. 

Given a train dataset $\mathcal{D}_{train}=\{(\mathbf{x}_i,y_i)\}_{i=1}^N$, the posterior is modeled by the classifier $h(\mathbf{x}, \theta_h)$. There exists an optimal target classifier $h_{t}$ and its corresponding $p_{t}(Y|\mathbf{X})$ for the balanced evaluation metrics. To approximate $p_{t}(Y|\mathbf{X})$, we usually obtain an $p_m(Y|\mathbf{X})$ via the learned classifier $h_m(\cdot)$ based on the $\mathcal{D}_{train}$.

To achieve this goal, one straightforward strategy is to minimize the expectations of  KL-divergence between $p_{t}(Y|\mathbf{X})$ and $p_{m}(Y|\mathbf{X})$ on $\mathcal{D}_{train}$, as follows:
\begin{align}
	& &\underset{\Theta}{\text{min}} 
	& & & \underset{\mathcal{D}_{train}}{\mathbb{E}}\{\mathcal{KL}(p_t(Y|\mathbf{X}))||p_m(Y|\mathbf{X})\}\\
	&\approx &\underset{\Theta}{\text{min}} 
	& & &  \frac{1}{N}\sum_{i=1}^N\mathcal{KL}(p_t(Y|\mathbf{x}_i)||p_m(Y|\mathbf{x}_i))\label{eq:goal_1}
\end{align}
as the first term $p_t(Y|\mathbf{x}_i)\log(p_t(Y|\mathbf{x}_i))$ of Eq.\ref{eq:goal_1}, is a constant, the Eq.\ref{eq:goal_1} is equivalent to
\begin{align}
	& &\underset{\Theta}{\text{min}} 
	& & &-\frac{1}{N}\sum_{i=1}^Np_t(Y|\mathbf{x}_i)\log(p_m(Y|\mathbf{x}_i))\\%\label{eq:goal_1}
	&\Leftrightarrow &\underset{\Theta}{\text{min}} 
	& & & -\frac{1}{N}\sum_{i=1}^N\left[ \sum_{y\in\mathcal{C}}p_t(y|\mathbf{x}_i)\log(p_m(y|\mathbf{x}_i))\right]\label{eq:goal_2}	
\end{align}
We can reformulate $p_t(y|\mathbf{x}_i)$ in Eq.\ref{eq:goal_2} with a $\delta(\cdot)$ function as:
\begin{align}
	p_t(y|\mathbf{x}_i)=\sum_{c\in \mathcal{C}} w_c\cdot\delta_c(y|\mathbf{x}_i)\label{eq:goal_3}
\end{align}
where $w_c$ is the class-wise coefficient of the target posterior, and we typically have $w_c=1$ for each class in a unbiased $\mathcal{D}_{train}$.

Substituting formulas (\ref{eq:goal_3}) into formula (\ref{eq:goal_2}), our optimization object can be written as:
\begin{align}
%	& &\underset{p(\mathbf{X})}{\text{min}} 
%	& & & -\frac{1}{N}\sum_{i=1}^N\left[ \sum_{y\in\mathcal{C}}w_c\cdot\log(p_m(y|\mathbf{x}_i))\right]\label{eq:goal_4}\\
%	&\propto & \underset{p(\mathbf{X})}{\text{min}} 
	& & \underset{p(\mathbf{X})}{\text{min}} 
	& & & -\frac{1}{N}\sum_{i=1}^N\left[ \sum_{y\in\mathcal{C}}w_c\cdot\log\left(\exp(y\cdot(\mathbf{w}_j^\intercal\mathbf{x}_i))\right)\right]\label{eq:goal_5}\\
	&= & \underset{p(\mathbf{X})}{\text{min}} 
	& & & -\frac{1}{N}\sum_{i=1}^N\left[ \sum_{y\in\mathcal{C}}w_c\cdot\left(y\cdot(\mathbf{w}_j^\intercal\mathbf{x}_i)\right)\right]
\end{align}
Now optimization goal for one input $\mathbf{x}$ with label $c_j$  is equivalent to:
\begin{align}
	\mathcal{L}=-w_c\cdot\log\left(\frac{\exp(z_j)}{\sum_{k=1}^C\exp(z_k)}\right)\label{eq:goal_6}
\end{align}
where $w_c$ is the label prior of the reference class distribution, $z_j$ is the $j$-th class prediction logit  for input $\mathbf{x}$.


%\paragraph{Adaptive Calibration Function}
\subsubsection{Architecture of Distribution Alignment\rev{(need to be revised)}}\label{subsubsec:disalign_method}

%In our DisAlign framework, the feature extractor $g$ and classifier $h$ are first optimized jointly without any re-balance strategies. Given the fixed feature extractor, our main focus is to adjust the decision boundary by using distribution alignment in a simple way. Below we first present our proposed instance-adaptive distribution alignment in  Sec.\ref{subsubsec:disalign_method}. Then we will introduce a generalized reweight strategy to learn the distribution alignment effectively in Sec.\ref{subsubsec:generalized_reweight}. 
%We will focus dot-classifier setting and use $h(\mathbf{x},\mathbf{W})$ in the remaining of this section for notation clarity.

In this work, we adopt a two-stage learning scheme for all visual recognition tasks, which consists of: \textit{1) a joint learning stage} and \textit{2) a distribution calibration stage}. 

The feature extractor $f(\cdot)$ and original classifier(denoted as $h_o(\cdot)$ for clarity) are jointly learned on imbalanced $\mathcal{D}_{train}$ in the first stage, where the original classifier $h_o(\cdot)$ is severely biased due to the imbalanced data distribution.  We use instance-balanced strategy to learn $f(\cdot)$ and $h(\cdot)$ in this work.

For the second stage, the all parameters of $f(\cdot)$ are frozen and we only focus on the classifier to adjust the decision boundary.
One idea in previous works(\textit{e.g}. cRT\cite{kang2019decoupling}) aims to achieve distribution alignment by discarding $h_o(\cdot)$ and learning a new target classifier $h_t(\cdot)$ with re-balance strategy(\textit{e.g}. class-balanced re-sampling).Nevertheless, the limited annotated data in the tail categories making the second stage optimization for new classifier suffer from the noisy and easy to overfit, which results in a sub-optimal performance. 

Thus, we keep the original $h_o(\cdot)$ and freeze its parameters in the second stage. Then a light-weight distribution align module including a \textit{adaptive calibration function} and a \textit{generalized re-weight strategy} is developed to calibrate the classification scores. 

%Thus,  and is introduced to align the class prediction based on the original class prediction generated by $h_o(\cdot)$. 

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/exp_scale_illustration}
    	\vspace{-0.8cm}
    \caption{The left axis(red dotted line) denotes the category frequency $r_i$ and the right axis denotes the reweight coefficient at different scale$\epsilon$ on ImageNet-LT dataset.}
    \label{fig:exp_scale_illustration}
\end{figure}
\paragraph{Adaptive Calibration Function.}
We first propose a adaptive calibration function to achieve the flexible and confidence-aware distribution alignment for each data point.
For input $\mathbf{x}$, it's $j$-th class score prediction is defined as follows:
\begin{align}
	\hat{z}_j =& \sigma({\mathbf{x}})\cdot\left(\alpha_j\cdot\mathbf{w}_j^\intercal\mathbf{x} + \beta_j\right) + (1-\sigma({\mathbf{x}}))\cdot \mathbf{w}_j^\intercal\mathbf{x}\\
%	=& (1+\sigma({\mathbf{x}})(\alpha_j-1))\cdot \mathbf{w}_j^\intercal\mathbf{x} + \sigma({\mathbf{x}})\cdot\beta_j\\
	\Leftrightarrow & (1+\sigma({\mathbf{x}})\alpha_j)\cdot \mathbf{w}_j^\intercal\mathbf{x} + \sigma({\mathbf{x}})\cdot \beta_j\\
	=& (1+\sigma({\mathbf{x}})\alpha_j)\cdot z_j + \sigma({\mathbf{x}})\cdot \beta_j \label{eq:final}
\end{align}
where $\sigma({\mathbf{x}})$ is the instance-aware confidence estimation module, which is implement by a linear layer followed with a non-linear activation function(\textit{e.g.} sigmoid function) for all input $\mathbf{x}$,
$\alpha_j$ and $\beta_j$ is learnable parameter for each class to calibrate the prediction distribution. It's worth noting that the $\mathbf{w}_j$ is loaded from $h_o(\cdot)$ and keeps fixed during our distribution alignment stage. We only optimize the parameters of $(1+\sigma(\mathbf{x})\alpha_j)$ and $\sigma{\mathbf{x}}\cdot\beta_j$.


%In this work, we formulate such a two-stage idea as \textit{representation-learning-with-distribution-alignment}(denoted as \textbf{DisAlign}) framework for long-tail recognition tasks.
%

\paragraph{Generalized Re-weight Strategy.}%\label{subsubsec:generalized_reweight}
To achieve the effective distribution alignment discussed before, we need to introduce the label distribution prior $w_c$ in Eq.\ref{eq:goal_6}.
Re-balance strategy is an effective solution to introduce the label distribution prior. Typically, a class-balanced re-weighting term that is inversely proportional to the number of samples is added to the loss functions, which is used in many previous works. Inspired by the reweight with effective number of class\cite{cui2019class} strategy, we propose a generalized form of re-weight to model the distribution prior in a more flexible manner.

Specifically, we introduce a generalized reweight strategy to incorporate the label prior into $w_c$ as:
\begin{align}
		w_{c_j}= \frac{(1/r_j)^\epsilon}{\sum_{k=1}^C (1/r_k)^\epsilon}
%		\mathcal{L}&=-\frac{(1/r_j)^\epsilon}{\sum_{k=1}^C (1/r_k)^\epsilon}\cdot\log\left(\frac{\exp(\hat{z}_j)}{\sum_{j=1}^C\exp(\hat{z}_k)}\right)
\end{align}
where $r_i$ is the empirical class frequencies on the training set, $\epsilon$ is the scale hyper-parameter of our proposed generalized form. When $\epsilon=0$, the generalized reweight can be viewed as instance-balance rewegiht, and it will be converted into a class-balanced reweight by setting $\epsilon=1$. We plot the curve of reweight coefficients based on ImageNet-LT dataset in Figure \ref{fig:exp_scale_illustration} to illustrate our proposed generalized rewegiht method.  

Equipped with adaptive calibration function and generalized re-weight strategy, now the Eq.\ref{eq:goal_6} can be rewritten as:

\begin{align}
		\mathcal{L}&=-\frac{(1/r_j)^\epsilon}{\sum_{k=1}^C (1/r_k)^\epsilon}\cdot\log\left(\frac{\exp(\hat{z}_j)}{\sum_{j=1}^C\exp(\hat{z}_k)}\right)
\end{align}
%\begin{align}
%	w_i&=\frac{1}{r_i^p}\\
%	\hat{w}_i &= C\cdot\frac{w_i}{\sum_{j=1}^C w_j}\\
%	&=C\cdot\frac{r_i^{-p}}{\sum_{j=1}^C r_j^{-p}}\\
%	&=C\cdot\frac{n_i^{-p}/N^{-p}}{\sum_{j=1}^C (n_j^{-p}/N^{-p})}\\
%	&=C\cdot\frac{n_i^{-p}}{\sum_{j=1}^C n_j^{-p}}
%\end{align}
%\subsection{An Unified View for the Long-tail Recognition}\label{subsec:distribution_mismatch}


%\begin{table*}[]
%\caption{\textbf{Comparison with Related Methods.} $\lambda$ is the hypper-parameter, $\mathbf{x}$ is an input vector, $\mathbf{e}$ is the mean feature of the training data, $\mathbf{w}_i$ is the classifier parameter for $i$-th class.}
%\vspace{-0.8em}
%\centering
%\begin{tabular}{l|c|c|c|c|c}
%\toprule
%\multirow{2}{*}{Method}           & \multirow{2}{*}{Classifier} & \multicolumn{4}{c}{Align Method}\\
%\cmidrule{3-6}
% & & Type &  Re-Balance  & Magnitude & Margin   \\
%\midrule
%Joint             & Dot-Product &  -           &   -   & -          & -        \\\hline
%LWS\cite{kang2019decoupling}               & Dot-Product & Learnable    & CB-Resample & $\alpha_i$        &             0                \\
%$\tau$-Normalized\cite{kang2019decoupling} & Dot-Product & Hand-Craft   & CB-Resample & $1/||\textbf{w}_i||^\tau$   & 0         \\
%%$\tau$-Normalized & Dot-Product & Hand-Craft   & $\frac{1}{||w||^\tau}$   & 0       &     \\
%Logit Adjustment\cite{menon2020long}  & Dot-Product & Hand-Craft   & -           & 1.0        &   $-\lambda\log(r_i)$      \\
%Deconfound$^*$\cite{tang2020long}        & Cosine Similarity & Hand-Craft & -   & 1.0        &   $-\lambda d(\mathbf{x},\mathbf{e})\mathbf{w}_i^\intercal \mathbf{e}$    \\
%\midrule
%\textbf{DisAlign}   & Dot-Product       & Learnable & Generalized Reweight           & $1+\sigma(\mathbf{x})\alpha_i$        &   $\sigma(\mathbf{x})\beta_i$    \\
%\textbf{DisAlign$^*$}  & Cosine Similarity & Learnable & Generalized Reweight             & $1+\sigma(\mathbf{x})\alpha_i$        &   $\sigma(\mathbf{x})\beta_i$    \\
%\toprule
%\end{tabular}
%\label{tab:comparision_recent}
%\end{table*}

%The other strategies, like Logit Adjustment\cite{menon2020long}, Deconfound\cite{tang2020long} and $\tau$-normalized\cite{kang2019decoupling}, introduce the heuristic calibration post-processing to align the posterior distribution without learning a new classifier. To 


%\begin{align}
%& \underset{x}{\text{minimize}}
%& & f_0(x) \\
%& \text{subject to}
%& & f_i(x) \leq b_i, \; i = 1, \ldots, m.
%\end{align}
% Typically, the classifier is learned on the imbalanced $\mathcal{D}_{train}$, which results in the estimated posterior distribution is biased by the imbalanced data distribution(denoted as $p_{i}(Y|\mathbf{X})$). 
% However, such an target classifier is difficult to acquired due to we are unable to access the balanced dataset directly. The performance degradation in current long-tail system is mainly induced by the mismatch of the distribution $p_{i}(Y|\mathbf{X})$ and $p_{t}(Y|\mathbf{X})$. 


%We aim to obtain optimal performance with a balanced metric for unseen data, thus our learning purpose is to make the model estimated distribution(denoted as $P_e(X,Y)$) as close as the underlying distribution of the problem(denoted as $P_b(X,Y)$). 
%Therefore, in an ideal case, we expect:
%\begin{align}
%	P_e(X,Y) \approx P_b(X,Y)
%\end{align} 
%
%In practical scenario, we are able to access the train dataset $\mathcal{D}_{train}=\{(\mathbf{x}_i,y_i),\dots,(\mathbf{x}_N,y_N)\}$ with a distribution $P_{t}(X,Y)$, which is sampled from the underlying true distribution $P_b(X,Y)$.

%If the train dataset is uniformly sampled from the $P_b(X,Y)$(in our case, train dataset is balanced dataset), which means we have:
%\begin{align}
%	P_t(X,Y)\approx  P_b(X,Y)\label{eq:target_approx}
%\end{align}
%our optimization function can be formulated as:
%\begin{align}
% \min D_{KL}(P_b(X,Y)||P_e(X,Y))	\approx \\ \min D_{KL}(P_t(X,Y)||P_e(X,Y))
%\end{align}
%In practice, $D_{train}$ is given, it's equivalent to minimize the cross-entropy.
%
%However, $D_{train}$ is not sampled uniformly and biased by the head classes, resulting in an imbalanced version, Eq.\ref{eq:target_approx} is not hold, we need to introduce a calibrated $\hat{P}_t(X,Y)$ as an accurate approximation of $P_b(X,Y)$.
%Our optimization function is converted as:
%\begin{align}
%	\min D_{KL}(P_b(X,Y)||P_e(X,Y))\approx \\ \min D_{KL}(\hat{P}_t(X,Y) || P_e(X,Y))\\
%	=\min \sum_{\mathbf{x}\in X}\sum_{y\in Y}\hat{P}_t(X,Y)\log(\hat{P}_t(X,Y)))- \\
%	 \sum_{\mathbf{x}\in X}\sum_{y\in Y}\hat{P}_t(X,Y)\log(P_e(X,Y))\\
%	=\min - \sum_{\mathbf{x}\in X}\sum_{y\in Y}\hat{P}_t(X,Y)\log(P_e(X,Y))\\
%	=\min - \sum_{\mathbf{x}\in X}\sum_{y\in Y} \hat{P}_t(Y|X)\hat{P}(X)\log(P_e(Y|X)P_e(X))
%\end{align}

%
%\begin{align}
%	P_{o}(Y|X) = \frac{P_{o}(X,Y)}{P_{o}(X)}\\
%	P_i(Y|X)=\frac{P_i(X,Y)}{P_i(X)}
%\end{align}
%
%\begin{align}
%	\frac{P_{o}(Y|X)}{P_{i}(Y|X)}&=\frac{P_o(X,Y)}{P_o(X)}\cdot\frac{P_i(X)}{P_i(X,Y)}\\
%	&\approx \frac{P_o(X,Y)}{P_i(X,Y)}
%\end{align}
%\begin{align}
%	P_{o}(Y|X)\approx\frac{P_o(X,Y)}{P_i(X,Y)}\cdot P_i(Y|X)
%\end{align}
%where $P_o$ is the distribution modeled by the optimal model, $P_i$ is the distribution learned on the imbalanced train set $\mathcal{D}_{train}$
%\begin{align}
%	\frac{p_{i}(y|\mathbf{x})}{p_{o}(y|\mathbf{x})}&=\frac{p_{i}(\mathbf{x}|y)p_{i}(y)}{p_{i}(\mathbf{x})}\cdot\frac{p_{o}(\mathbf{x})}{p_{o}(\mathbf{x}|y)p_{o}(y)}\\
%	&\approx \frac{p_{i}(\mathbf{x}|y)p_{i}(y)}{p_{o}(\mathbf{x}|y)p_{o}(y)}
%\end{align}

%\begin{align}
%	\frac{p_{i}(y|\mathbf{x})}{p_{o}(y|\mathbf{x})}&=\frac{p_{i}(\mathbf{x}|y)p_{i}(y)}{p_{i}(\mathbf{x})}\cdot\frac{p_{o}(\mathbf{x})}{p_{o}(\mathbf{x}|y)p_{o}(y)}\\
%	&\approx \frac{p_{i}(\mathbf{x}|y)p_{i}(y)}{p_{o}(\mathbf{x}|y)p_{o}(y)}
%\end{align}
%One straightforward idea is estimating a precise classifier $h_{e}$ to approximate $h_{o}$ by incorporating class distribution prior, where the class prediction predicted with $h_{e}$ is denoted as $p_{e}(y|\mathbf{x})$.

% to align these two mismatched distributions by minimize the KL-divergence of these two distributions based on the class prior. We denote the class prediction of $h^{ali}$ on $\mathbf{x}$ as $p_{ali}(C)$

%\begin{align}
%&\min\quad KL(P_{o}(Y|X)||P_{e}(Y|X))=\sum_{\mathbf{x}\in X}\sum_{y=c_i}^{c_k}p_{o}(y|\mathbf{x})\log{\frac{p_{o}(y|\mathbf{x})}{p_{e}(y|\mathbf{x})}}\\
%&=\sum_{y=c_i}^{c_k}p_{o}(y|\mathbf{x})\log{p_{opt}(y|\mathbf{x})} - \sum_{y=c_i}^{c_k}p_{o}(y|\mathbf{x})\log{p_{e}(y|\mathbf{x})}\\
%&\propto \min  - \sum_{y=c_i}^{c_k}p_{o}(y|\mathbf{x})\log{p_{e}(y|\mathbf{x})}\\
%& = \max \sum_{y=c_i}^{c_k}p_{o}(y|\mathbf{x})\log{p_{e}(y|\mathbf{x})}
%\end{align}

%\begin{align}
%\min\quad & D(p_{opt}(C)||p_{ali}(C)) \\ 
%&\propto  \min - \sum_{\mathbf{x}\in\mathbf{X}}p_{opt}(C)\log{p_{ali}(C)}\\
%&\propto \max \sum_{\mathbf{x}\in\mathbf{X}}p_{opt}(C)\log{p_{ali}(C)} 	
%\end{align}
%
%\begin{align}
%\min\quad & D(p_{opt}(y|x)||p_{ali}(y|x)) \\ 
%&\propto  \min - \sum_{\mathbf{y_i}\in\mathbf{C}}p_{opt}(y|x)\log{p_{ali}(y|x)}\\
%&\propto \max \sum_{\mathbf{y_i}\in\mathbf{C}}p_{opt}(y|x)\log{p_{ali}(y|x)} 	\\
%&\propto \max \sum_{\mathbf{y_i}\in\mathbf{C}}p_{opt}(y|x)\log({\mathbf{W}_{ali}^\intercal\mathbf{x}})
%\end{align}


%\begin{align}
%p_{imb}(C|X)=\frac{p_{imb}(X|C)p_{bal}(C)}{p_{imb}(X)}\\
%p_{bal}(C|X)=\frac{p_{bal}(X|C)p_{bal}(C)}{p_{bal}(X)}
%\end{align}

%\begin{align}
%&\text{minimize.}\quad D(p_{bal}(y)||p_{imb}(y))\\
%&=\sum_{x\in\mathbf{X}}p_{bal}(c_i)\log{\frac{p_{bal}(c_i)}{\hat{p}_{imb}(c_i)}}\\
%&=\sum_{x\in\mathbf{X}}p_{bal}(c_i)\log{p_{bal}(c_i)} - \sum_{x\in\mathbf{X}}p_{bal}(c_i)\log{\hat{p}_{imb}(c_i)}\\
%&\propto  - \sum_{x\in\mathbf{X}}p_{bal}(c_i)\log{\hat{p}_{imb}(c_i)}	
%\end{align}

%We model the posterior of the classifier with the \textit{Bayes' theorem} as:
%\begin{align}
%	\hat{y}_i = \hat{\mathbf{w}}_i^\intercal\mathbf{x}+b_i=\alpha_i\mathbf{w}^\intercal\mathbf{x} + \beta_i
%\end{align}
%Learn a high-dimensional classifier with only a few annotated available for tail categories is challenging and easy to overfitting, thus we simplify the model by only learning the magnitude $\alpha$ and margin $\beta$ based on the score predicted by the original $h_{i}$ learned in the representation learning stage. This could also be considered as an implicit regularization. Furthermore, we also introduce a confidence estimation term to achieve instance-aware distribution alignment as follows:
%\begin{align}
%%	\hat{y}_i &= \sigma(\mathbf{x})\cdot(\alpha_i\mathbf{w}^\intercal\mathbf{x} + \beta_i) + (1-\sigma(\mathbf{x}))\cdot\mathbf{w}^\intercal\mathbf{x}\\
%	\hat{y}_i &= (1+\sigma(\mathbf{x})\alpha_i)\cdot\mathbf{w}_i^\intercal\mathbf{x}+\sigma(\mathbf{x})\beta_i
%\end{align} 
%where $\mathbf{w}_i$ is the original parameter of the original classifier and is fixed during the DisAlign. $\sigma(\cdot)$ is the confidence estimation function. $\alpha_i$ and $\beta_i$ is the learnable magnitude and margin, respectively. 

%\begin{align}
%&\text{minimize.}\quad D(p_{bal}(c_i)||\hat{p}_{imb}(c_i))\\
%&=\sum_{x\in\mathbf{X}}p_{bal}(c_i)\log{\frac{p_{bal}(c_i)}{\hat{p}_{imb}(c_i)}}\\
%&=\sum_{x\in\mathbf{X}}p_{bal}(c_i)\log{p_{bal}(c_i)} - \sum_{x\in\mathbf{X}}p_{bal}(c_i)\log{\hat{p}_{imb}(c_i)}\\
%&\propto  - \sum_{x\in\mathbf{X}}p_{bal}(c_i)\log{\hat{p}_{imb}(c_i)}
%\end{align}

%Our optimization goal is :
%\begin{align}
%	&\text{maximize.} \sum_{x\in\mathbf{X}}p_{bal}(c_i)\log{\hat{p}_{imb}(c_i)}
%\end{align}

%\subsection{Representation: Object-aware Feature Learning}
\begin{table}[]
\caption{\textbf{Comparison with Related Methods.} $*$ means for cosine classifier, 'L' and 'H' means the learnable and hand-craft, 'CB-RS' is the class-balanced resampling, 'G-RW' is generalized reweight, $\lambda$ is the hypper-parameter, $\mathbf{e}$ is the mean feature of training data, $d(\cdot)$ is cosine distance.)}
%, $\mathbf{w}_i$ is the classifier parameter for $i$-th class.}
\vspace{-0.8em}
\centering
\resizebox{0.4999\textwidth}{!}{
\begin{tabular}{l|c|c|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}}          & \multicolumn{4}{c}{\textbf{Align Method}}\\
\cmidrule{2-5}
 & Type &  Balance  & Magnitude & Margin   \\
\midrule
Joint            &  -           &   -   & -          & -        \\\hline
LWS\cite{kang2019decoupling}               & L   & CB-RS & $\alpha_i$        &             0                \\
$\tau$-Normalized\cite{kang2019decoupling}  & H   & CB-RS & $1/||\textbf{w}_i||^\tau$   & 0         \\
%$\tau$-Normalized & Dot-Product & Hand-Craft   & $\frac{1}{||w||^\tau}$   & 0       &     \\
Logit Adjust\cite{menon2020long}  & H   & -           & 1.0        &   $-\lambda\log(r_i)$      \\
Deconfound$^*$\cite{tang2020long}        & H & -   & 1.0        &   $-\lambda d(\mathbf{x},\mathbf{e})\mathbf{w}_i^\intercal \mathbf{e}$    \\
\midrule
\textbf{DisAlign}      & L   & G-RW           & $1+\sigma(\mathbf{x})\alpha_i$        &   $\sigma(\mathbf{x})\beta_i$    \\
\textbf{DisAlign$^*$}    & L & G-RW             & $1+\sigma(\mathbf{x})\alpha_i$        &   $\sigma(\mathbf{x})\beta_i$    \\
\toprule
\end{tabular}}
\label{tab:comparision_recent}
\end{table}


\begin{table*}[h!]
\centering
\caption{\textbf{Quantitative results on ImageNet-LT:} All models use the feature extractor trained with 90 epoch(except the last two row), $*$ means the model uses cosine classifier. 
\textbf{R-50} and \textbf{X-50} means the ResNet-50 and ResNeXt-50, respectively.}
\vspace{-0.8em}
% \begin{threeparttable}
 \resizebox{0.85\textwidth}{!}{
\begin{tabular}{l|c|l|lll|l|lll}
\toprule
\multirow{2}{*}{\textbf{Method}}  & \multirow{2}{*}{\textbf{Align}} & \multicolumn{4}{c|}{\textbf{Top-1 Accuracy@R-50}} & \multicolumn{4}{c}{\textbf{Top-1 Accuracy@X-50}}  \\
\cmidrule{3-10}
                                  &             &\textbf{Average} & \textbf{Many } & \textbf{Medium  } & \textbf{Few  } &\textbf{Average} & \textbf{Many  } & \textbf{Medium  } & \textbf{Few  } \\
\midrule
Baseline    & -           & 41.6	           & 64.0           &    33.8         &  5.8           & 44.4	          & 65.9           &       37.5     &  7.7 \\
Baseline$^*$                   & -               & 48.4  & 68.4   &  41.7    & 15.2                 & 49.2   & 68.9   &  42.8  & 15.6\\
%Cosine                            & -           & 48.4             &  68.4          &    41.8         &  15.2          & 49.2        &  68.9               &    42.8     & 15.6\\
\midrule
NCM\cite{kang2019decoupling}          & \multirow{4}{*}{ Hand-Craft }  & 44.3             & 53.1           &    42.3         &  26.5         & 47.3         & 56.6          &        45.3    &   28.1\\
$\tau$-Norm\cite{kang2019decoupling}  & & 46.7             & 56.6           &    44.2         &  27.4         & 49.4         & 59.1          &        46.9    &   30.7    \\
Logit Adjust\cite{menon2020long}                   &   & 50.3             & -              &      -          &   -           &            - & - &- &-\\
Deconfound$^{*}$\cite{tang2020long}           &    &  -               & -              &      -          &   -           & 51.8            & 62.7       &        48.8    &   31.6\\
%\cmidrule{2-2}
\midrule
cRT\cite{kang2019decoupling}           &  \multirow{5}{*}{Learnable}  & 47.3             & 58.8           &    44.0         &  26.1         &  49.6        & 61.8          &        46.2    &   27.4\\
cRT$^{*}$\cite{kang2019decoupling} &   & -                & -              &    -            &   -           &  49.7        & 60.4          &        46.8    &   29.3\\
LWS\cite{kang2019decoupling}          &   & 47.7             & 57.1           &    45.2         &  29.3         &  49.9        & 60.2          &        47.2    &   30.3  \\
%Naive$^\dagger$   & - & 45.2        &  67.4               &    38.0    & 7.5  \\
%Cosine$^\dagger$  & - & R-50 & 48.4        &  68.4               &    41.8    & 15.2   \\
%Naive-Bound                           &  -          & 56.1             & 62.3           &   53.6          & 47.6\\
\cmidrule{1-1}\cmidrule{3-10}
\textbf{DisAlign}                     &   &  51.3\more{(+1.0)}  &  59.9  &  49.9   &  31.8      
                                                    &  52.6\more{(+0.8)}  &  61.5 &  50.7  &  33.1\\
\textbf{DisAlign$^{*}$}           &   &  52.9\more{(+2.6)}   &  61.3  &  52.2   &  31.4
												    &  53.4\more{(+1.6)}  &   62.7  &  52.1   &  31.4\\
%\midrule
%\textbf{DisAlign$^{*}$}               &  Learnable   &  53.7\more{(+3.4)}  &   63.1  &  51.5  &  34.7     
%													 &  54.4\more{(+2.6)}  & 65.0  & 51.6 & 34.4  \\
%\textbf{DisAlign$^{\dagger *}$}       &  Learnable   &  53.6\more{(+3.3)}  &   64.0 &   51.7  &  30.9     & \\
%\midrule
%cRT+SSP  & Learnable & 51.3 & - \\
%\midrule
%\textbf{DisAlign + SSP} & Learnable\\
%\textbf{DisAlgin$^{\dagger}$ + SSP} & Learnable\\
%\textbf{DisAlign$^\dagger$}\small(F-200e)   &  Learnable  &  \textbf{52.7} & 65.2 & \textbf{49.7} & 27.6 \\
%\midrule
%Naive$^\dagger$     & - & 45.2        &  67.4               &    38.0    & 7.5  \\
%Naive+SA$^\dagger$     & - & 48.4        &  68.4               &    41.7    & 15.5  \\
%\textbf{DisCal-Naive}  & & R-50 &  Learnable     &  51.7 & 62.3 & 48.7 & \textbf{32.1}   \\
%\textbf{DisCal-Cosine} & & R-50 &  Learnable  &  \textbf{52.7} & 65.2 & \textbf{49.7} & 27.6 \\
%\midrule
%cRT$^\dagger$\cite{kang2019decoupling}   & Learnable& 52.8   &   65.8  & 49.1 & 28.9  \\
%Cosine\cite{} & X-50 & 47.6 & 67.3 & 41.3 & 14.0\\
%\midrule
%Naive$^\dagger$   & X-50     & 46.8        &  68.1               &    40.2    & 9.3   \\
%Cosine$^\dagger$  & X-50     & 49.2        &  68.9               &    42.8    & 15.6  \\
\bottomrule
\end{tabular}} %\end{threeparttable}
\label{tab:imagenet_lt}
\end{table*}

\subsection{Connection with Recent Works}
Below we dicuss the connections between our proposed distribution alignment strategy and recent two-stage works. Detailed comparison is reported in Table \ref{tab:comparision_recent}.

Logit Adjustment\cite{menon2020long} and Deconfound\cite{tang2020long} introduce a hand-craft margin to adjust the distribution while keep the magnitude as 1.0, and incorporate the class prior directly in $r_i$ or $\mathbf{w}_i$ without re-training. LWS\cite{kang2019decoupling} and $\tau$-normalized\cite{kang2019decoupling} try to achieve the similar goal by learning a magnitude scale and discard the margin adjustment. 

All these methods can be considered as the special cases of our DisAlign approach,
%, either typicall which heavily depend on the dataset prior and limits the model capacity for the complex high-dimensional feature representation. 
which provides a unified and simple form to model the distribution mismatch in a learnable way. 
Moreover, the resample based strategy is not easy to be applied for the instance-level(object detection/instance segmentation) or pixel-level(semantic segmentation) tasks, our generalized reweight provides an alternative solution to incorporate the class prior in a simple and effective manner. Experimental results in Sec \ref{sec:exp} also demonstrate our method compared with aforementioned works.

\subsection{Learning and Inference}\label{subsec:learning_inference}
Our method is a generic solution for various long-tail problem, and we will present the instantiation of DisAlign in various visual recognition tasks in this section. 
%\subsubsection{Learning on Different Vision Tasks}
Following a two-phase learning scheme, we first learn the feature extractor $g$ and classifier $h$ jointly in the first stage. 
\paragraph{Image Classification and Semantic Segmentation}
For the image classification and semantic segmentation, the feature extractor and initial classifier is fixed, we only learn two class-wise magnitude and margin parameters, along with the parameter of instance-aware confidence estimation module in second stage. 
In the inference process, the classification score is first predicted with the default model, followed by a classification prediction adjustment with DisAlign as Eq.\ref{eq:final}.

\paragraph{Object Detection and Instance Segmentation}
Similarly, the same strategy is also valid for object detection and instance segmentation. We first learn the standard detection model(\textit{e.g.} Mask R-CNN\cite{he2017mask}) in the first stage. Then all networks are fixed and we only learn the magnitude, margin and confidence estimation module. The second-stage learning process is easy to be optimized and typically requires a small overhead. Different with image classification the generalized reweight is only applied for the foreground categories in training loss.

For the inference, box location, mask prediction and classification score are also first predicted with the default model, followed by a classification prediction adjustment as Eq.\ref{eq:final}.



==> sections/related.tex <==
\section{Related Works}


%\subsection{Imbalance Learning} 
\subsection{Re-balancing based Methods}
To alleviate the adverse effect caused by long-tail distribution in visual recognition, resample-based methods and reweight-based methods have been extensively studied.

%The basic thinking of resample-based methods is over-sampling the minority categories or under-sampling the frequent categories in the training process\cite{buda2018systematic}. Class-aware sampling\cite{shen2016relay} proposes to choose samples of each category equiprobably in the training batch, which is a widespread idea used for many vision tasks\cite{liu2019large, gao2018solution}. Repeat factor sampling \cite{mahajan2018exploring} is a smoothed sampling method conducting repeated sampling for tail categories, which is applied in \cite{gupta2019lvis} and boost the performance on instance segmentation significantly. In addition, \cite{wang2019data} proposes to increase the sampling rate for categories with low performance after each training epoch and balances the feature learning for under-privileged categories.

The basic thinking of resample-based methods is over-sampling the minority categories or under-sampling the frequent categories in the training process\cite{buda2018systematic}. Class-aware sampling\cite{shen2016relay} proposes to choose samples of each category equiprobably, which widely used for many vision tasks\cite{liu2019large, gao2018solution}. Repeat factor sampling \cite{mahajan2018exploring} is a smoothed sampling method conducting repeated sampling for tail categories, which is applied in \cite{gupta2019lvis} and effective on instance segmentation. In addition, \cite{wang2019data} proposes to increase the sampling rate for categories with low performance after each training epoch and balances the feature learning for under-privileged categories.


An alternative strategy is to re-weight the loss function, \cite{huang2016learning} propose to re-weight the plain loss with category-specific coefficients inverse with the sample distributions, which is equivalent to adjust the learning rate for each category. Further, \cite{cui2019class} defines the effective samples number for each target category and redesigns the coefficients negative correlated with the effective samples number. However, the one-stage re-balancing based methods achieve the limited successes due to sub-optimal representations

%Recent works \cite{xiang2020learning}, \cite{chu2020feature},\cite{Jamal_2020_CVPR}
\subsection{Few-shot Learning} 
Our work is also related to the few-shot learning. The early works focus on the metric learning and attempt to learn feature representations that preserve the class neighborhood structure. Matching Network\cite{vinyals2016matching} employs a differentiable nearest neighbor classifier implemented with an attention mechanism over the learned representations. Prototypical Network\cite{snell2017prototypical} learns to classify the query image by computing distances to prototype feature vectors of the novel categories. In addition, feature hallucination\cite{hariharan2017low} and augmentation\cite{wang2018low} are also effective to boost the performance. However, these methods often suffer a moderate performance drop for head classes since they mainly focus on novel classes. While the goal of long-tail visual recognition is to maintain high performance on head and tail categories simultaneously, which is different with few-shot learning only concerning about the novel categories.

More recent works\cite{gidaris2018dynamic, ren2018incremental} attempt to remedy this issue by utilizing the duality between features and classifiers’ weights\cite{qi2018low,qiao2018few}. \cite{qi2018low} exploits the symmetry between normalized features and weights in classification network and proposes to directly imprint the weights for tail categories by coping the embedding activation for the corresponding exemplar. However, these methods usually use a balanced dataset of the novel classes.


\subsection{Visual Recognition Tasks} 
Visual recognition community has witnessed significant progress with deep convolutional networks in recent years. Object detection, instance segmentation and many other challenging visual recognition tasks have been actively studied in plenty of works.
Image object detection is a core vision task, and a common branch is R-CNN\cite{girshick2014rich} based method, which detects objects based on the region proposals. Fast R-CNN\cite{girshick2015fast} proposes to extract the whole image feature once to reduce the computation cost of R-CNN. Faster-RCNN\cite{ren2015faster} introduces a region proposal network that share the same backbone with the detection to build the first unified end-to-end efficient network for object detection. Mask R-CNN\cite{he2017mask} extends Faster R-CNN by adding a branch for predicting the object masks in parallel with the existing branch for bounding box recognition.

